Foliated Open Books

This paper introduces a new type of open book decomposition for a contact three-manifold with a specified characteristic foliation $\mathcal{F}_\xi$ on its boundary. These \textit{foliated open books} offer a finer tool for studying contact manifolds with convex boundary than existing models, as the boundary foliation carries more data than the dividing set. In addition to establishing fundamental results about the uniqueness and existence of foliated open books, we carefully examine their relationship with the partial open books introduced by Honda-Kazez-Matic. Foliated open books have user-friendly cutting and gluing properties, and they arise naturally as submanifolds of classical open books for closed three-manifolds. We define three versions of foliated open books (embedded, Morse, and abstract), and we prove the equivalence of these models as well as a Giroux Correspondence which characterizes the foliated open books associated to a fixed triple $(M, \xi, \mathcal{F})$.

==> background.tex <==
% !TEX root = FOB_main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Contact structures and open books} 
\vv{reading 24/09} \jel{So we agree we'll remove this?  The subsection abotu equivalence should go somewhere else, although I'm not sure what's natural.  Otherwise, we can put careful references in the introduction for open books, abstract OBs, and convex surfaces.}
Throughout the paper, we consider orientable three-manifolds with co-orientable contact structures.  It's well established that open book decompositions are one of the most effective means to study such contact manifolds, and we recalls some definitions  and notation here. Readers are referred to \cite{Geiges, Etnyre} for further discussion of the basic objects.


\subsection{Open books}\label{sec:ob}
In 
\begin{definition}\label{def:eob} $(B,\pi)$ is an \emph{open book} for \vv{a closed manifold} $M$ if $B$ is an oriented link in $M$, $\pi:M\setminus B\rightarrow S^1$ is a fibration, and $B=\partial \left(\pi^{-1}(t)\right)$ for all $t\in S^1$. The link $B$ is called the \emph{binding} of the open book and the closure $\overline{\pi^{-1}(t)}$ of each fiber is called a \emph{page}.
\end{definition}


\begin{definition} An open book $(B, \pi)$ \emph{supports} a contact form $\alpha$ if $\alpha (TB)>0$ and if $d\alpha|_{\pi^{-1}(t)}$ is an area form for all $t\in S^1$.  An open book supports a contact structure $\xi$ if $\xi$ is isotopic through contact structures to the kernel of some $\alpha$ supported by $(B,\pi)$
\end{definition} 


The following results are classical and fundamental:

\begin{theorem}[\cite{Etnyre}]  Every open book supports a unique isotopy class of contact structure.
\end{theorem}

\begin{theorem}[\cite{Etnyre}]  Every contact structure is supported by some open book.
\end{theorem}

The structure defined in Definition~\ref{def:eob} is sometimes known as an honest or embedded open book to distinguish it from the following:
\marginpar{\vv{I never heard honest open book for these, and we wanted to reserve it for "open book for closed manifold"}}
\begin{definition} An \emph{abstract open book} is $(S, h)$, where $S$ is a surface with boundary and $h\in \text{Diff}^+(S)$ such that $h|_{\vv{N(\partial S)}}=\text{Id}$. \marginpar{\vv{If you don't glue in a solid torus near the binding, then you need to have the identity in a neighbourhood}}
\end{definition}

The data of an abstract open book determines a closed three-manifold $M(S,h)$ as follows:
\[ M(S,h)= \frac{S\times [0,1]}{\sim}\]
where ``$\sim$'' denotes two equivalences: 
\begin{itemize}
\item for all $x\in S$, $(x, 1)\sim \big(h(x), 0)$; and
\item for all $x\in \partial S$, $t, t'\in [0,1]$, $(x, t)\sim (x, t')$.
\end{itemize}

The diffeomorphism type of the manifold constructed from $(S,h)$ depends only on $[h]\in \text{Mod}(S)$, and the notation $(S,h)$ is often used to denote $M(S,h)$ itself. \vv{There is a natural embedded open book decomposition on $M(S,h)$ given by $B(S,h)=\partial S\times\{t\}$ (these are identified for all $t$) and $\pi(S,h)\vert_{\mathring{S}\times {t}}=t$. An embedded open book $(B,\pi)$ on $M$ is described (?) by the abstract open book $(S,h)$ if there is a diffeomorphism between $M(S,h)$ and $M$ that takes $(B(S,h),\pi(S,h))$ to $(B,\pi)$. The abstract open books that describe the same embedded open books are related to each other by conjugation of $h$ by a diffeomorphism of $S$.}

\begin{definition} \vv{An abstract open book $(S,h)$ \emph{supports} the contact structure $\xi$ on $M(S,h)$ if $(B(S,h),\pi(S,h))$ supports $\xi$.}
\marginpar{ \jel{Torisu def or via diffeo to honest open book?  This choice should reflect what we do later}}
\end{definition}
\vv{Or equivalently we can phrase this using a reformualtion of Torisu \cite{Torisu}. An open book decomposition $(S,h)$ gives rise to a Heegaard decomposition of $M(S,h)$ with the handlebodies $U=S\times[0,1/2]/\sim$ and $V=S\times [1/2,1]/\sim$} \marginpar


\subsection{Equivalence}
In the main portion of the paper, we will introduce several notions of foliated open books and establish precise relationships between them.  We thus find it advantageous to be explicit about the equivalence between abstract and honest open books in closed case.  A common slogan is that honest open books are defined up to isotopy, while abstract open books are defined only up to diffeomorphism.  However, there is a  further equivalence on honest open books required for the correspondence with the abstract models. 

Suppose that $p:S^1\rightarrow S^1$ is a diffeomorphism of $S^1$ and that $(B, \pi)$ is an open book for a manifold $M$. Then $p\circ \pi$ has the same level sets (``pages'') as $\pi$, but a priori $(B, p\circ \pi)$ is not an open book, as it does not have the right model near the binding. In order to achieve the ``right model'' near the binding we need to modify $p\circ \pi$ in $N(B)\cong B\times D^2_{\varepsilon}$ as follows. Let $\Psi_{\varepsilon/2}^\varepsilon$ be a smooth bump function that is 0 for $r\ge \varepsilon$ and 1 for $r\le \varepsilon$. Define

\begin{equation*}
p(\pi) = \left\{
\begin{array}{ll}
 \Psi_{\varepsilon/2}^\varepsilon(r)\vartheta+(1-\Psi_{\varepsilon/2}^\varepsilon(r)p(\vartheta)) & \text{if } r\le \varepsilon,\\
\pi\circ p & \text{if } r> \varepsilon.
\end{array} \right.
\end{equation*}
This function is clearly smooth, and the local model for open books works in $B\times D_{\varepsilon/2}^2$. This also means that this type of reparametrizataion does not affect the infinitesimal local model, so we will often ignore it.  

The smooth contact manifold constructed from  the data of an opem book is only well defined up to such reparatmeterization, so it must be invoked as an additional equivalence on honest open books in order to move freely between the honest and abstract cases.   



%Then $(B, p \circ \pi)$ is again an open book, and it's clear that the level sets on any surface ---the intuitive interpretation of the open book foliation--- will agree.   Away from the elliptic points, we have $d(p \circ \wtpi)= dp(\wtpi) d\pit$. %compute $d (q\circ \pit)=d(\pit^*q)=\pit^* dq$.  
% Since $dp(\pit)>0$ is a multiple of a volume form, it suffices to note that it is a positive multiple and  we see that the associated $1$-forms differ by a positive function, so the equivalence class of the foliation is preserved. Nevertheless, the local model imposed near the elliptic points requires some work before these two may be naturally identified. 
 
%\vv{Let $\F=(E,\pit, H=H_+\cup H_-)$ be an open book foliation, and consider an orientation preserving diffeomorphism $p\colon S^1\to S^1$. We would like to obtain a new foliation $p(\F)$, with the same singular points $E,H=H_+\cup H_-$, but with the leaves reparametrised using the function $p$. }







==> comments.tex <==
% !TEX root = FOB_main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Embedded OBD is wrong: reparameterisation is never in it. (Need the reparameterisation, and we should include this. 

in def of dividing set, distinguish between OB foliation, where it's defined up to isotopy and char foliation where it depends on the choice of convex vector field

\vv{-this is not a major issue, but we have to explain what we mean when we write $d\pi\wedge d\alpha$, as $\pi$ is a map to $S^1$ (not to R), so $d\pi$ is a map between $T\Sigma$ and $TS^1$, we probably should lift everything to the universal cover $R\to S^1$, but then we will have trouble with the notation, as we already use tilde for the restrictin of $\pi$ to $\Sigma$. Let's just in general check if everything we write makes sense, maybe we can add a remark in the begining, once we really understand what's going on (but now i have the same issue when I try to set up the open book for reparametrisation..)}

\vv{Use $A\!\smallsetminus\!B$ instead of $A\setminus B$}

\vv{04.10: I am thinking about introducing two notations for foliations to separate characteristic foliations and open book foliations. What about $\F$ and $\mathcal{G}$?}

\vv{04.10: $g$ is not a good letter for reparametrizing $\pi$. What about $p\colon S^1\to S^1$?}

\vv{Let's decide if we should put circle free somewhere earlier, it's quite annoying to write it all the time, but I am happy with any solution except that we cannot add it to OBF definition, as that's not how others are using it..}\jel{I think we can put it earlier, but we're still going to want to include it in the statement of the theorems, so that someone just skimming the results will get the correct version.}


\vv{before we start to write properly we need to decide how much we go into details about foliations. I want to be more honest about things, but if we only need to change $\Fob$s around elliptic points to match the definition, and then never use it later, then maybe it's not worth it}

\vv{Does the usage of $S^1$-Morse foliation really simplify things? how confusing would it be to use open book foliation for any tuple $(\pit,E,H=H_+H_-)$ with $\pit\colon \Sigma\!\smallsetminus\! E \to S^1$, local ... near $E, H$ saddle points.... ?Independently whether it comes form an embedding or not. We prove very early that anything like that can be obtained by an embedding..}

\vv{choose vs chose }\jel{??} \vv{that was a note for me, I think I mixed the two at some cases..}

\jel{neighbourhood vs neighborhood: I'm happy with either American or Commonwealth spellings, but I'd prefer to be consistent (so neighbourhood -> colour, centre, etc.). Until this draft, I think it's all been American.}

\vv{$\Fob$ vs $\F_\pi$}\jel{I think these have been used for slightly different things; $\Fob$ is specifically the open book foliation, i.e., the intersecton of a surface with pages of an honest open book.  (I realise these are leaves, not vector fields, but that's a separate issue.) $\F_\pi$ is the foliation by level sets of $\pi$, where $\pi$ might not be a regular function.  I think it's okay to conflate these to simplify the notation, but we should say so if we do that.}

\vv{Should we paramtrize a circle with [0,1] or with $[0,2\pi]$, I choose $[0,1]$ earlier, mostly because I already used $\pi$ for the map in the open book, and I didn't want anyone to be confused..} \jel{[0,1]}

\vv{sorry for this mess, I copy-paste here something you wrote about gradient-like vectorfields:}
then we can define the ascending and descending manifold of each boundary critical point.  A smooth vector field is gradient-like for $\wtpi$ if its zeroes occur exactly at the singular points of $\mathcal{F}$ and if it is  positively transverse to $\mathcal{F}$ away from the singular points. \vv{I still think that we need more than this, the behaviour near the 0's is important. Giroux uses the notion pseudo gradient (in French, so it might be different), but it says: $X\cdot f\ge \rho |df|^2$ where $\rho$ is a positive function}. Any such vector field can be extended to a vector field which is gradient-like for $\pi$. \jel{Need proof?  Is this true?} \vv{Probably true, the idea should be that gradient-like vectorfields form a  convex set, and you can construct them with partition of unity.. We have to think it through, but don't need to write it down.}\jel{for reference, probably remove later:} %https://arxiv.org/pdf/1207.3066.pdf

\begin{enumerate}
\item $X\cdot \pi >0$ away from critical points of $\pi$
\item near each boundary critical $p$ on $\partial M=\{x_2=0\}$, in the neighborhood  $\{x_2\geq 0\}$ we have
\[ \pi(x_1, x_2, x_3)=\pi(p)-x_1^2\mp x_2^2+x_3^3\]
and 
\[ X=(-x_1, \mp x_2, x_3)\]
\item $X$ is tangent to $\partial M$.
\end{enumerate}


With respect to such a vector field, we can identify the ascending and descending manifolds of each critical point $p$.  Letting $\gamma_p(s)$ denote the point in $M$ to which $p$ flows after time $s$, we write
\[W_p^\pm= \{  x\ |\  p=\lim_{s\rightarrow \pm \infty} \gamma_x(s) \}.\]
The descending manifold of $p$ is synonymous with $W_p^+$, while the ascending manifold is $W_p^-$.  Note that when $p$ is a boundary critical point of index $k$, the dimension of $W_p^+$ is $k$.  
%\vv{Can we name everything? Like ascending/descending manifolds and ... $W_p^\pm$, $S_p^\pm(t)=W_p^\pm\cap \pi^{-1}(t)$}
\vv{end of copy-paste}


\subsection{\jel{Older embedded stuff}}

\begin{lemma}\vv{Will we use this?} Let be a neighborhood of the union of the descending gradient flow lines from any  positive hyperbolic point with critical value less than $t$; 
the ascending gradient flow lines from any  negative hyperbolic point with critical value less than $t$; and  the leaf $\wtpi^{-1}(t)$:
\[R_t=\big[ \bigcup_{\text{ind}(p)=2, \pi(p)<t} N(W_p^+)\big] \cup \big[\bigcup_{\text{ind}(p)=1, \pi(p)<t} N(W_p^-)\big] \cup \big[ N(\wtpi^{-1}(t) )\big].\]
\jel{I put in the proper notation, but I prefer the version without it.}
Then $R_t$ is homeomorphic to $R^+$. 
\end{lemma}\begin{proof} (Easy to see this for $t=0$, then show passing through a hyperbolic point preserves the neighborhood.)\end{proof}



We begin by interpreting the condition that an embedded foliated open book for $(M, \xi)$ is sorted in terms of a corresponding abstract foliated open book.  Fix a diffeomorphism respecting the decomposition into pages from $(B, \pi, \F_\pi)$ to $(\{S_i\}, h)$.  This map carries the set $W_p^+\!\smallsetminus\!  \pi^{-1}[-\epsilon, \epsilon]$ to a set of   discs embedded disjointly in $M \!\smallsetminus\!  \pi^{-1}[-\epsilon, \epsilon]$.  If $p$ is an index 1 critical point on the handlebody $\partial H_i$, then the corresponding ascending manifold maps to a disc that intersects $H_j$ for $j\geq i$.  Similarly, for an index 2 $q\in \partial H_i$, the image of $W_q^-\!\smallsetminus\!  \pi^{-1}[-\epsilon, \epsilon]$ maps to a disc that intersects $H_j$ for $j\leq q$.  For $i\neq 0, 2k$, let $S_i'$ be the abstract page formed by cutting along arcs of intersection between $S_i$ and the set of imported $W_q^-$ and $W_p^+$. 




\begin{proposition}\label{prop:makepfob}  The surfaces $S'_i$ and $S'_j$ are homeomorphic for $i, j\in \{1, \dots, 2k-1\}$ and the triple $(S_0, S'_1, h)$ defines a partial open book embedded in and contactomorphic to the original $(M, \xi)$.  
\end{proposition}



\begin{proof}[Proof of Proposition~\ref{prop:makepfob}] 
(1) each change in the topology of a page has been pushed either forward or backward to happen at the transition between $0$ and $1$ or $2k-1$ and $2k$, so the topology of the page is constant for $t\in [\epsilon, 2\pi-\epsilon]$.

(2) To see that the new  manifolds embeds in the original one, note that there is a pagewise embedding of the uncollapsed abstract POB $(S_0, S'_1, h)$ into the  original FOB $(\{S_i\}, h)$. 

The remainder of this proof is dedicated to showing that the POB represents a contactomorphic submanifold of the original.  To do so, we continue to view the partial open book as being embedded pagewise in the original foliated open book, and we define an isotopy from $\partial M$ to the boundary of the embedded partial open book through convex surfaces  with isotopic dividing sets.  It follows that the original and final manifolds differ only by a manifold contatomorphic to $\partial M \times I$ with an $I$-invariant contact structure, and thus are contactomorphic. 

Since $\partial M$ is convex, it has an $I$-invariant neighborhood.  Let $\Sigma$ denote a parallel copy of $\partial M$ in this neighborhood.  Note that $\Sigma$ is disjoint from the critical points of the original function $\pi$.  Second, note that the gradient-like vector field $\nabla \pi$ is contact and transverse to $\Sigma$ in a neighborhood of $\coprod_{i,j}W_{p_i}^+\cup W_{q_j}^w-$.  \jel{WHY? Is the point that for an abstract open book, $\partial_t$ is contact, and choosing $\nabla \pi$ is essentially like parameterising the manifold so that this is $\partial_t$? I understand that we can choose a metric to realise a vector field satisfying some essentially topo conditions, but saying we have this flexibility for the contact structure seems like it needs more justification.* }  

Consider first an intersection of $\Sigma$ with some $W_p^+$. Push  $\Sigma$ along the flowlines of $\nabla \pi$ in a neighborhood of $\Sigma\cap W_p^+$until it reaches $S_{1-\epsilon}$.  Then in the manifold bounded by $\Sigma$ but not $\partial M$, all the pages in $\pi^{-1}( \pi(p), 1-\epsilon)$ have been cut along the ascending manifold of $p$, as required in the construction described above.  On the other hand, $\Sigma$ remains transverse to the contact vector field $\nabla \pi$ throughout the isotopy and we may see directly that the dividing set changes only by isotopy during the deformation.  It follows that the resulting manifold differs from the original only by a product neighborhood of $\partial M$, and hence is contactomorphic.

\jel{Hmm, I though we could claim $\Gamma$ changes only by isotopy, but I now think I just drew the picture (IMG\_6695) so that this works.  What do we know about the characteristic hypersurface inside a half-handle?  Perhaps this ties into * above and requires an explicit contact model of the handle. }

Repeat this process for each critical point until each page $S'_i$ has been cut out of $S_i$ by $\Sigma$. As noted above, the result is a manifold diffeomorphic \marginpar{\jel{homeo yes, diffeo not justified yet}} to $M$ and equipped with the structure of a partial open book, and it follows from the construction of the gradient-like vector field in Figure~\ref{fig:grad} that the dividing set associated to the partial open book is isotopic to the dividing set on $\Sigma$.  


\end{proof}



\vv{This is subsection 4.6.2, but I hate to scroll all the time, so I edit it here, do not read yet!}


\subsubsection{Layer for reparametrisation}\label{sssec:layer} \vv{Do not read yet}

Here we describe a trivial open book for the reparametrization of an open book foliation $\F=(\pit,E,H=H_+\cup H_-)$ with an orientation preserving diffeomorphism of  $p\colon S^1\to S^1$. As earlier let $g(\F)=(g(\pit),E,H=H_+\cup H_-)$, and remember, that $g(\pit)$ differs from the composition $g\circ \pit$ \vv{Maybe we should use a different notation..} only around the elliptic points. As in subsection \ref{sec:egcircle}, we define a 1-form $\beta'=g\beta$ for $\pit$, and a contact structure given by $\alpha=\beta'+fdz$. We will use an ``open book decomposition'' for the manifold $\Sigma\times I$, (in this case by an ``open book'' for a manifold with boundary we simply mean a pair $(B,\pi)$ so that $B$ is properly embedded $\alpha(TB)>0$ and $d\alpha$ is an area form with respect to the pages, and $\pi\vert_{\Sigma\times \partial I}$) gives an open book foliation) and then change it near $\Sigma\times \partial I$ it as in Proposition \ref{prop:exp} to obtain a foliated open book.

As in subsection  \ref{sec:egcircle} let $B=E\times I$ with orientation $\pm\partial z$, depending on the sign of the elliptic point. Let $\pit_z=(1-z)\pit+zg(\pit)$, and define the function
\[\pi=\pit_z+fz\]
on $\Sigma\times [0,1]\!\smallsetminus\! B\colon S^1$.
Then, as in the calculations of Proposotion \ref{}, we have that $\pi$ is an ``open book decomposition'' supporting $\ker\alpha$ if and only if 
\[\omega'=d\pit_z\wedge df+(f+\dot\pit_z)d\beta'\]
is an area form on $\Sigma$, where $\dot\pit_z=\partial/\partial z\pit_z$. With the choices in Proposition \ref{} this is an area form if $|\dot\pit_z|<1$. Computing 
\[\dot\pit_z=g(\pit)-\pit<1,\]
as $S^1$ is of length 1. \vv{this again, secretly happens in the lift of the maps to $\R$}



Let $\beta'=g\beta$ be the 1-form corresponding to $\pit$ as in Lemma \ref{lem:approx}. Recall, that in the construction $\beta$ agrees with $d\pit$ away from the neighbourhoods of $E\cup H$, in a disc-neighbourhood $D^2(r\vartheta)$ of $e\in E$, the 1-form $\beta$ is obtained from $d\pit=\vartheta$ by multiplication with $r^2$ and a bump function, while in the neighbourhood of $H$ we added a bump-function times $xdy$ in coordinates, where $\pit=x^2-y^2$. 

In the following we try to understand how we can get these 1-forms for the reparametrised open book foliation $\F_1=p(\F)=(\pit_1=p(\pit),E,H=H_+\cup H_-)$. Away from the singular points $E\cup H$, we have $\beta_1=d\pit_1=d(p\circ\pit)=(\dot{p}\circ \pit)d\pit=(\dot{p}\circ \pit)\beta$.

Near a hyperbolic point $h\in H$ we again have $d\pit=(\dot{p}\circ \pit)d\pit$, and in the coordinates $(x,y)$ near $h$ as above we get $d\pit=(\dot{p}\circ \pit(x,y))$

 Near an elliptic point we sl

 First, let $e\in E_\pm$, it has a neighbourhood $D^2(r,\vartheta)$, where $\pit=\vartheta$. Here, we have to change the foliation 


and the function $g$ depends only on the flow of $\F$. In the neighbourhood of $E$ $\beta$ is obtained from $d\pit$ by multiplication with $r^2$ and a bump function, while in the neighbourhood of $H$ we added $ydx$




First notice, that if $g\beta$ is the 1-form corresponding to $\pit$ as in Lemma \ref{lem:approx}, then $gp'(\pit)\beta$ gives gives a 1-form, that corresponds to $p\circ \pit$. Indeed, all one needs to check is that $p'(\pit)\beta$ agrees with $d(p\circ \pit)=p'(\pit)d\pit$ away from the neighbourhoods of $E\cup H$ and that $d(p'(\pit)\beta)$ has the right sign at $E_\pm\cup H_\pm$  \vv{check ???}

$\pit_z$ for $z\in [0,1]$ just reparametrisation
and corresponding $\beta'_z=g\beta_z$ ($g$ only depends on the foliation, so we can assume it's the same. $f$ only depends on $\Gamma$ )
\[\alpha=g\beta_z+Cfdz,\]
For sufficiently large $C$ $\alpha$ will be a contact structure
\[\alpha\wedge d\alpha=(g\beta_z+Cfdz)\wedge(dg\wedge\beta+gd\beta_z+(g\dot{\beta_z}+Cdf)\wedge dz)=\]
\[=dz\wedge\left(g^2\beta_z\wedge \dot{\beta_z}+Cg\beta_z\wedge df +Cfdg\wedge\beta_z+Cfg d\beta_z\right)\]

So \[g^2\beta_z\wedge \dot{\beta_z}+Cg\beta_z\wedge df +Cfdg\wedge\beta_z+Cfg d\beta_z>0\]

$\pi=\pit_z+Cfz$, \vv{Do I want the $C$ there?}
% then \[d\pi=d\pit_z+\dot{\pit}_zdz+Czdf+Cfdz\]
\[d\pi\wedge d\alpha=(d\pit_z+(\dot{\pit}_z+Cf)dz+Czdf)\wedge (dg\wedge\beta_z+gd\beta_z+(g\dot{\beta_z}+Cdf)\wedge dz)= \]
\[=dz\wedge\left((\dot\pit_z+Cf)(dg\wedge \beta_z+gd\beta_z)+gd\pit_z\wedge\dot\beta_z+Cd\pit_z\wedge df+Czgdf\wedge\dot\beta_z\right)\]

So we need \[(\dot\pit_z+Cf)(dg\wedge \dot\beta_z+gd\beta_z)+gd\pit_z\wedge\dot\beta_z+Cd\pit_z\wedge df+Czgdf\wedge\dot\beta_z>0\]
The difference on $\Sigma$: \vv{grrrr!!}

\[\dot\pit_z(dg\wedge \beta_z+gd\beta_z)\]

%\[=(gd\pit_z \wedge\dot{\beta_z} +Cd\pit_z\wedge df +Czgdf\wedge \dot{\beta_z} )\wedge dz\]

\vv{END of Do not read!}

\begin{proposition}[Expansion]\label{prop:ex} 
Let $(B,\pi)$ be an open book for the 3-manifold $M$ and 
let $\Sigma\subset M$ be a closed, oriented surface embedded in $M$ so that $(B,\pi)$ induces an open book foliation $\F_\pi$ with no circle leaves on $\Sigma$. Then there exists a contact structure $\xi$ on $M$ supported by $(B,\pi)$
so that $\Sigma$ is convex with respect to $\xi$ and its dividing curve $\Gamma$ divides $\F_\pi$. 
We can find a neighbourhood $N(\Sigma)\cong\Sigma\times [\varepsilon,\varepsilon]$ with $I$ invariant contact structure $\xi\vert_{N(\Sigma)}$ and an $S^1$-valued Morse function $\pi'\colon M\!\smallsetminus\! B\to S^1$ so that the following hold:
\begin{enumerate}
\item $\pi'$ is $C^0$ close to $\pi$ and agrees with $\pi$ outside of a neighbourhood of $N(\Sigma)$;
\item for any hyperbolic point $h_\pm\in H_\pm$ of $\F_\pi$ the function $\pi'$ has a pair of canceling critical points $p_{h_\pm}^\pm=h_\pm\times \{\pm\varepsilon\}\in\Sigma_\pm=\Sigma\times \{\pm \varepsilon\}$;
\item the index of $p_{h_\pm}^\pm\in \Sigma_\pm$ is $2$ if the sign of $h_\pm$ and $\Sigma_\pm$ agree, and $1$ otherwise;
\item $\pi'$ has no other critical points;
\item $\nabla \pi'\in T\Sigma_\pm$;
\item $\pi'$ defines an open book foliation $\F_{\pi'}^\pm=(\pi'\vert_{\Sigma_\pm},E\times \{\pm\varepsilon\},H\times\{\pm\varepsilon\}=H_+\times\{\pm\varepsilon\}\cup H_-\times\{\pm\varepsilon\})$ on $\Sigma_\pm$ that is topologically conjugate and \vv{$\delta$-isotopic} to $\F_\pi$ and is still divided by $\Gamma$. 
\end{enumerate} \qed
\end{proposition}
As we will see, the statement uses a local model for the neighbourhood of $\Sigma$ with a given open book foliation, thus the product manifolds $T_m^e=\Sigma\times[-\varepsilon,0]$ and $T_e^m=\Sigma\times[0,\varepsilon]$ together with the restricted bindings and Morse functions 
\[\left(B_m^e=\left(E_+\times [-\varepsilon,0] \right) \cup \left(E_-\times \overline{[-\varepsilon,0]}\right) ,\pi_m^e=\pi'\vert_{\Sigma\times[-\varepsilon,0]}\right)\] and 
\[\left(B_e^m=\left(E_+\times [0,\varepsilon] \right) \cup \left(E_-\times \overline{[0,\varepsilon]}\right) ,\pi_e^m=\pi'\vert_{\Sigma\times[0,\varepsilon]}\right)\] 
 are standard too. The Morse foliated open book for $T_m^m=\Sigma\times [-\varepsilon,\varepsilon]$ is given by 
 \[\left(B_m^m=\left(E_+\times [-\varepsilon,\varepsilon] \right) \cup \left(E_-\times \overline{[-\varepsilon,\varepsilon]}\right) ,\pi_m^m=\pi'\vert_{\Sigma\times[-\varepsilon,\varepsilon]}\right),\]
while $T_e^e=T_e^m\cup T_m^e$ is a priory not embedded into $M$.

First we prove of Proposition \ref{prop:exp}, and then proceed to show how these constructions relate embedded- and Morse foliated open books. 

\begin{proof}[Proof of Proposition \ref{prop:exp}]\vv{have not read this carefully for a while, check if it matches current notation..}

We start with the open book foliation $\Fob=(\pit,E,H=H_+\cup H_-)$ and use Corollary \ref{cor:lm} to choose a local model for the neighbourhood $N(\Sigma)\cong\Sigma(x,y)\times I(z')$ with $I=[-\eta,\eta]$. 
In this model, $B=E\times I$,  with orientation $\pm\partial z$ depending on the sign of each elliptic point, and $\pi=\pit+fz$, where $f$ is the function from Proposition \ref{prop:Gi} that is $\pm 1$ on $R_\pm'$ and monotonically increasing in $u$ on $A\cong N(\Gamma)$. For sufficiently small $\eta$, all surfaces $\Sigma\times \{z'\}$ ($z'\in[-\eta,\eta]$) have induced open book foliations topologically conjugate and \vv{$\delta$ isotopic} to $\Fob$. \marginpar{\vv{in applications, we wanted to cut along properly embedded surfaces (probably we want the boundary to be transverse to the foliation), to mirror partial gluing, and it might also be useful to cut along a surface that is embedded, but has a transverse boundary.. I think all of these should work with an extra model near the boundary, but the formulations get more complicated.. I will eventually include it.}}


We will modify $\pi$  near the singular points of  $\Fob$. First reparametrise the $I$ coordinate by $z$, where $z'=z^3+\rho z$ for some $\rho>0$. Note that $z\in [-\zeta,\zeta]$, where $\zeta^3+\rho\zeta=\eta$. Now define a path of functions $\pi_s$ that agrees with $\pi$ outside of a three-ball neighbourhood $B_{\varepsilon}^3(h)$ of each hyperbolic point $h\in H_\pm$ and that is defined as follows on $B_{\varepsilon}(h)$:
\[\pi_s=(1-\Psi_{\varepsilon/2}^{\varepsilon}(r))\pi+\Psi_{\varepsilon/2}^{\varepsilon}(r)(\pit+z^3-sz)=\pit+z^3+z(\rho-(s+\rho)\Psi_{\varepsilon/2}^{\varepsilon}(r)).\]
As before,   $\Psi_{\varepsilon/2}^{\varepsilon}$ is a smooth bump function that equals $1$ for $r< \varepsilon/2$ and $0$ for $r>{\varepsilon}$.
Remember that here $r$ is the distance from $h$ in $B_{\varepsilon}$; i.e., $r^2=x^2+y^2+z^2$.
Clearly $\pi_{-\rho}=\pi$, and we will show that $\pi_s$ is a regular function for $s<0$; it is non-Morse only for $s=0$,
 with an embryonic critical point at each hyperbolic point; and for $s>0$, it is Morse with two cancelling critical points of index 1 and 2 associated to each hyperbolic point $h$. In order to prove the previous claim, in the following we determine the critical points of $\pi_s$. Away from $D_{\varepsilon}(h)$, the function $\pi_s=\pi$ and is thus  is regular, while its differential on $D_{\varepsilon}(h)$ is
\[d\pi_s=d\pit+(3z^2+\rho-(s+\rho)\Psi_{\varepsilon/2}^{\varepsilon})dz-z(s+\rho)d\Psi_{\varepsilon/2}^{\varepsilon}dr\]

For $r>\varepsilon$ the $\Sigma$-component of  $d\pi_s$ equals $d\pit\neq 0$, thus $d\pi_s\neq 0$.
In the annulus $A=\{\varepsilon/2\le r\le\varepsilon\}$ observe that the coefficient of  $dx$ and the coefficient of $dy$ in $d\pit$ are $-2x$ and $2y$,  respectively, thus their proportion is $-x:y$. While in $z(s+\rho)d\Psi_{\varepsilon/2}^{\varepsilon}dr$ the proportion of the coefficients of $dx$ and $dy$ is $x:y$. This means that if in their sum both coefficients are 0, we must have $x=y=0$. Thus the possible critical points of $d\pi_s$ are all of the form $(0,0,z)$ with $\varepsilon/2\le z \le\varepsilon$. In these points the $dz$ coordinate of the equation $d\pi_s=0$ simplifies to:
\[3z^2+\rho-(s+\rho)\Psi_{\varepsilon/2}^{\varepsilon}-z(s+\rho)d\Psi_{\varepsilon/2}^{\varepsilon}=0\]
On $A$ we have $3z^2\ge \varepsilon^2/4$, while $\vert\rho-(s+\rho)\Psi_{\varepsilon/2}^{\varepsilon}\vert$ can be $<\varepsilon^2/8$ if we choose both $s$ and $\rho$ small. 
As for the third term,
\[-z(s+\rho)d\Psi_{\varepsilon/2}^{\varepsilon}\le\varepsilon/2(s+\rho)K,\] 
where $K=\max_{\varepsilon/4\le r\le\varepsilon/2}\{-d\Psi_{\varepsilon/2}^{\varepsilon}\}>0$. Thus if we choose $|s+\rho|$ sufficiently small we can ensure that this third term is $<\varepsilon^2/8$ and it follows that $d\pi_s$ is nonzero on A.

For $r<\varepsilon/2$ we have 
$d\pi_s=\d\pit+(3z^2-s)dz$. Thus for $\sqrt{\frac{s}3}<\varepsilon/2$,  there are critical points at $z=\pm \sqrt{\frac{s}3}$. 
 
 
In summary, for sufficiently small $\rho>0$ and $|s|$ the function $\pi_s$ is a Morse function for $s\neq 0$. It is regular whenever $s<0$, it has an embryonic critical point at the hyperbolic points $h$, and has a pair of cancelling index 1 and 2 critical points for each hyperbolic point $h$ on the surfaces $\Sigma\times\{\pm \sqrt{\frac{s}3}\}$.

In the following we will understand the singularities and the leaves of the foliation induced by $\pi_s$ on $\Sigma\times\{z\}$.
Notice, that if we restrict $\pi_s$ to $\Sigma\times\{z\}$, then we get a function $\pit+C$ (for $C=z^3-zs$) in $B_{\varepsilon/2}^3$ and $\pit+C'$ (for $C'=z^3+\rho z$) outside $B_{\varepsilon/2}^3$, thus the level sets of $\pit$ agree with the level sets of $\pi_s\vert_{\Sigma\times\{z\}}$ on $B_{\varepsilon/2}^3\cup\Sigma\!\smallsetminus\! B_{\varepsilon}^3 $. From the previous computation we have seen, that $\pi_s\vert_{\Sigma\times \{z\}}$ has no critical points on the annulus $A=\{\varepsilon/2\le r\le\varepsilon\}$. The arcs on $A$ connect the leaves $\pit^{-1}(a)$ on $D^2_{\varepsilon/4}$ to the leaves of $\pit(a-(\rho+s)z)$ of $\Sigma\!\smallsetminus\!\cup_h D^2_{\varepsilon/2}$. This means, that if we choose both $|z|$ and $|\rho+s|$ sufficiently small, the foliation induced by
 $\pi_s\vert_{\Sigma\times\{z\}}$ will be topologically conjugate to $\Fob$, moreover these changes can be made arbitrarily small, so for example we can achieve that the neighbourhoods of the associated positive graphs $G_{++}$ to the level sets of $\pit$ and $\pi_s\vert_{\Sigma\times \{z\}}$ agree. 

Now fix sufficiently small $s<0$ and $\rho>0$, so that all the above results hold and let $\pi'=\pi_s$, $\Sigma_\pm=\Sigma\times\{\pm \sqrt{\frac{s}3}\}$. Then we can cut $M$ along these two surfaces. Depending on whether $\Sigma$ was separating or not, we get two or three 3-manifolds that are the closures of $M\!\smallsetminus\! \left(\Sigma_+\cup\Sigma_-\right)$, one of which is $\Sigma\times [-\sqrt{\frac{s}3},\sqrt{\frac{s}3}]$ with boundary $-\Sigma_-\cup\Sigma_+$. 
 % In the case when $\Sigma$ is separating. Then the 3-manifolds after the cut are $M_1$ with boundary $\Sigma_-$, $M_3$ with boundary $-\Sigma_+$ and the middle one $M_2\cong\Sigma\times [-\sqrt{\frac{s}3},\sqrt{\frac{s}3}]$ with boundary $-\Sigma_-\cup\Sigma_+$. When $\Sigma$ is nonseparating, then apart from $M_2\cong\Sigma\times [-\sqrt{\frac{s}3},\sqrt{\frac{s}3}]$ we only have $M_1$ with boundary $\Sigma_-\cup-\Sigma_+$. 


To complete the proof of the stated result,  we  need to choose a model contact structure $\xi$ according to Corollary \ref{cor:lm}
so that  $\F_\xi$ on $\Sigma$ is divided by $\Gamma$, and $\xi$ is $I$-invariant in the neighbourhood. Then by choosing $s,\varepsilon$ and $\rho$ sufficiently small, we can get open book foliations $\F_{\pi'}^\pm$ on $\Sigma_\pm$ that are \vv{$\delta$-isotopic} to $\F_{\pi}$ for arbitrarily small $\delta$. We then choose $\delta$ small enough so that $\F_{\pi'}^\pm$ is still divided by $\Gamma$.
\end{proof}

%\jel{If some boundary component is a sphere foliated by parallel arcs, then there are no handles.  How do  the two different types of bigons connect the two elliptic points?}


Notice that the local model of Corollary \ref{cor:lm} used to prove Proposition~\ref{prop:exp} still applies in the interior of foliated open books, so we get the following:
\begin{proposition}[Cutting]\label{prop:cut}
Let $(B,\pi,\F)$ be a foliated open book for a  3-manifold $(M,\F)$ with foliated boundary and 
let $\Sigma\subset M$ be a closed oriented surface embedded in $M$ so that $(B,\pi)$ induces an open book foliation $\F_\pi$  on $\Sigma$ with no circle leaves. Then there exists a contact structure $\xi$ on $M$ supported by $(B,\pi,\F)$
so that $\Sigma$ is convex with respect to $\xi$ and its dividing curve $\Gamma$ divides $\F_\pi$. 

Furthermore, there exists a neighbourhood $N(\Sigma)$ of $\Sigma$ and a\jel{n $S^1$-valued} Morse function $\pi'$ on $M$ and a gradient-like vectorfield $\nabla\pi'$ for $\pi'$ such that 
%Furthermore, there exists a neighbourhood $N(\Sigma)$ of $\Sigma$ and a Morse function $\pi'$ such that 

\begin{enumerate}
\item $\pi'$ is $C^0$ close to $\pi$ and agrees with $\pi$ outside of a neighbourhood of $N(\Sigma)$;
\item for any hyperbolic point $h_\pm\in H_\pm$ of $\F_\pi$ the function $\pi'$ has a pair of canceling critical points $p_{h_\pm}^\pm=h_\pm\times \{\pm\varepsilon\}\in\Sigma_\pm=\Sigma\times \{\pm \varepsilon\}$;
\item the index of $p_{h_\pm}^\pm\in \Sigma_\pm$ is $2$ if the signs of $h_\pm$ and $\Sigma_\pm$ agree, and $1$ otherwise;
\item $\pi'$ has no other critical points;
\item  $\nabla \pi'\in T\Sigma_\pm$; 
\item $\pi'$ defines an open book foliation $\F_{\pi'}^\pm=(\pi'\vert_{\Sigma_\pm},E\times \{\pm\varepsilon\},H\times\{\pm\varepsilon\}=H_+\times\{\pm\varepsilon\}\cup H_-\times\{\pm\varepsilon\})$ on $\Sigma_\pm$ that is topologically conjugate and \vv{$\delta$-isotopic} to $\F_\pi$ and is still divided by $\Gamma$. 
\end{enumerate}
This means that $(B\cap N(\Sigma),\pi'\jel{|_{N(\Sigma)}},\F_{\pi'}^+\cup \F_{\pi'}^-)$ is a trivial  foliated open book %\vv{(i.e.\ the local model..)} 

for $(N(\Sigma),\xi\vert_{N\jel{(\Sigma)}}, -\F_{\pi'}^+\cup \F_{\pi'}^-)$, and \[(B^\Sigma=B\cap M^\Sigma,\pi^\Sigma=\pi'\vert_{M^\Sigma},\F^\Sigma=\F\cup \F_{\pi'}^+\cup -\F_{\pi'}^-)\] is a foliated open book for $(M^\Sigma=\overline{M\!\smallsetminus\! N(\Sigma)},\F^\Sigma)$. \qed 
\end{proposition}

\jel{Near the elliptic points,   the obvious change of $\pit=\vartheta$ to $p\circ \pit=\vartheta$ does not immediately work, as the angular extension of a diffeomorphism of $\partial D^2=S^1$ to $D^2$ need not be a diffeomorphism.  Instead, we modify the leaves slightly in a small neighbourhood $N(e)\cong D^2_\varepsilon(r,\vartheta)$ of each elliptic point $e\in E$ as follows.  Let $\Psi_{\varepsilon/2}^\varepsilon$ be a smooth bump function that is $0$ for $r\ge \varepsilon$ and 1 for $r\le \varepsilon/2$%Take a path $p_t$ of orientation preserving diffeomorphisms of $S^1$ from $p_0=\id_S^1$ to $p_1=p$. Then c
Then the homeomorphism $P\colon D^2_\varepsilon\to D^2_\varepsilon$
\[P(r,\vartheta)=\left(r,\Psi_{\varepsilon/2}^\varepsilon(r)p(\vartheta)+\left(1-\Psi_{\varepsilon/2}^\varepsilon(r)\right)\vartheta\right),\]
 is smooth. Thus if we change $p\circ \pit$ to $\Psi_{\varepsilon/2}^\varepsilon(r)\vartheta+\left(1-\Psi_{\varepsilon/2}^\varepsilon(r)\right)p(\vartheta)$ in $N(e)$, then we get a function $p(\pit)$ that gives an open book foliation $p(\F)=(E,p(\pit), H=H_+\cup H_-)$, that we call the \emph{reparametrisation} of $\F$. We will generally consider open book foliations up to such reparameterization; we write $\F_{ob}=(E,[\pit], H=H_+\cup H_-)$ to denote the associated equivalence class and $\F_{\pi}=(E,\pit, H=H_+\cup H_-)$ when we consider a specific representative. }



==> ctctfob.tex <==
% !TEX root = FOB_main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{From contact 3-manifolds to Foliated Open books}

The main result of this section is that stabiliztaion allows us to  put all foliated open books in a standard form. 
  
\begin{theorem}\label{thm:decomp} After possibly stabilizing a foliated open book, it may be decomposed \vv{What do we mean by this?, that they are glued together??} as a partial open book and a product partial foliated open book.
\end{theorem}

\vv{This is part of Prop 8.4.}
\vv{We should rephrase it afterwards.}
We prove this theorem in two steps.  The first step describes a topological condition between cutting arcs  and attached handles on the pages of a foliated open book $(B, \pi, \mathcal{F})$.  Proposition~\ref{prop:makepfob} establishes that when this condition is satisfied, there is a natural way to identify a partial open book inside and contactomorphic to the original manifold.  The second step (Proposition~\ref{prop:disj}) shows that this condition may be achieved via a sequence of positive stabilizations.  An important consequence of Theorem~\ref{thm:decomp} is the following Giroux Correspondence for foliated open books.


\begin{theorem}[Giroux Correspondence] Suppose that $(B_1, \xi_1, \mathcal{F})$ and  $(B_2, \xi_2, \mathcal{F})$ are foliated open books for contactomorphic manifolds with the same boundary foliation.  Then there exists a sequence of positive (de)stabilizations taking $(B_1, \xi_1, \mathcal{F})$ to  $(B_2, \xi_2, \mathcal{F})$.
\end{theorem}

\jel{And we should say how we change the foliations}


\begin{proof} After possibly stabilizing, Theorem~\ref{thm:decomp} may be applied to decompose $(B_i, \xi_i, \mathcal{F})$  into a partial open book $M(S_i, P_i, h_i)$ for contactomorphic manifolds and a product partial foliated open book.  Applying the Giroux Correspondence for partial open books, we get the existence of a sequence of positive (de)stabilizations taking $M(S_1, P_1, h_1)$ to $M(S_2, P_2, h_2)$.  This yields the desired sequence of (de)stabilizations for the corresponding foliated open books.
\end{proof}



\section{Applications}

(all speculative)

bordered sutured contact invariant in HF

partial gluing (hasn't been published by HKM)

some examples for manifolds without known OBs, cut-and-paste, \dots

explain IK moves?
\section{Questions}

Given a surface separated into $R_\pm$, what is the minimal number of singular points needed to equip it with a compatible $S^1$ foliation?

Does there exist a set of moves between all the compatible $S^1$ foliations for a fixed $\Gamma$?

Are these moves realizable as a result of gluing FOBs for balls?

Strong versus weak compatibility for characteristic and open book foliations (perhaps layers do this?)

What's the proper way to say what kind of foliations are $S^1$ compatible? (strong and  weak versions, depending on whether we're considering a supported contact structure or just a topological object)





\jel{I think everything after this is notes that belong in a draft folder, not in the paper, although we may want to use bits and pieces.  Do you see any content we need after this?  (1/19)}



%*********************************************************************************************

==> modelsuv.tex <==
% !TEX root = FOB_main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Local Models } \label{sec:models}

\jel{I don't like the fact that the orientation changes from $(u,v,z)$ to $(v,u)$; this is either notationally sloppy or actually a problem, and I'm trying to figure out which.}

This is a  technical section that may be skipped at first reading. As a start, we provide a neighborhood theorem for open book foliations on surfaces in Section~\ref{sec:nhood}, and we construct an explicit model for this neighborhood in Section~\ref{sec:egcircle}. Taken as a whole, this section lays the groundwork for moving between embedded, Morse, and abstract open books.   Such  freedom will be extensively employed in the rest of the paper, but on first pass, the reader may wish to focus only on  the results  in Section~\ref{sec:fobequiv} which describe the precise notions of equivalence between embedded, Morse, and abstract foliated open books.

\subsection{Neighborhood Theorem}\label{sec:nhood}
The key theorem is an extension to open book foliations of the usual neighborhood theorems for characteristic foliations. 
\begin{proposition}[Neighborhood Theorem]\label{prop:nbrh} 
Let $(B,\pi)$ and $(B',\pi')$ be open books for the 3--manifolds $M$ and $M'$ respectively. Let $\Sigma\hookrightarrow Y$ and $\Sigma'\hookrightarrow Y'$ be embedded surfaces with induced open book foliations $(\F_{\pit}, \pit,H=H_+\cup H_-)$ and $(\F_{\pit}',\pit', H'=H'_+\cup H'_-)$. Suppose that there is a diffeomorphism $\psi\colon \Sigma\to \Sigma'$ that takes the two open book foliations to each other; i.e., $\psi(E)=E'$, $\pit'\circ\psi=\widetilde{\pi}$, and $\psi(H_\pm)=H_\pm'$. Then there are neighborhoods $N=N(\Sigma)$ and $N'=N(\Sigma')$ and an extension of $\psi$ to $\Psi\colon N\to N'$ so that 
\begin{enumerate}
\item $\Psi(B)=B'$;
 \item $\pi=\pi'\circ\Psi$;
 \item $\Psi(B\cap N)=B'\cap N'$ and the trivialisation of $N(B)\cap N\cong (B\cap N)\times D^2$ in which $\pi=\vartheta$ is mapped by $\Psi$ to the trivialisation of $N(B')\cap N'\cong (B'\cap N')\times D^2$ in which $\pi'=\vartheta$. %
 \end{enumerate}
Moreover, one can choose supported contact structures $(M,\xi)$ and $(M',\xi')$ for $(B,\pi)$ and $(B',\pi')$,  respectively, so that $\Psi$ is a contactomorphism between $(N,\xi\vert_{N})$ and $(N',\xi'\vert_{N'})$. 
\end{proposition}





\begin{proof}
Let us first describe local models around the points of $\Sigma\subset Y$. For each point $p\in {\Sigma}$ we will give a neighborhood $D_p^2\times I$ of $p$ in $Y$ with coordinates adapted to $(B,\pi)$. These coordinates are chosen by a repeated use of the Implicit Function Theorem, and both the neighborhood $D_p^2$ and the interval $I$ might shrink as we make our additional choices. 

In the neighborhood of a \emph{regular point} $p$ of the foliation ${\F}_{\pi}$ we can choose local coordinates $(\jel{v,u},z)$ on $Y$ so that $\jel{v}=\pi-\pit(p)$, ${\Sigma}=\{z=0\}$ with orientation $(\partial \jel{v},\partial \jel{u})$ and coorientation $\partial z$, and the foliation ${\F}_{\pi}$ is directed by $\partial \jel{u}$. We call such a coordinate system in neighborhood that only contains regular points of ${\F}_{\pi}$ an \emph{adapted coordinate system}. The set of adapted coordinates in a given neighborhood $U$ is convex.

Around an \emph{elliptic point} $e_\pm$ of ${\F}_{\pi}$, we know that $B\pitchfork {\Sigma}$ at $e_\pm$, and $N(B)\cong B(\varphi)\times D^2(r,\vartheta)$. In these coordinates, $e_\pm=(\varphi_0,0,0)$, and in a sufficiently small neighborhood we can write $\Sigma\cap N(B)$ as the graph of a function $f\colon \{\varphi_0\}\times D^2\to \R$ that fixes $\{\varphi_0\}\times\{0\}$. Since $\Sigma$ is transverse to $B$ we have $df\neq d\varphi$ at the origin of $\{\varphi_0\}\times D^2$, so we can use the Implicit Function Theorem to choose coordinates $(z=f-\varphi$, $r,\vartheta)$. In these coordinates $\Sigma=\{z=0\}$, $B$ is oriented by $\partial z$, $\Sigma$ is cooriented by $\pm\partial z$, and $\pi=\vartheta$.



In a neighborhood of a hyperbolic point $h_\pm$,  the function $\pit=\pi\vert_{{\Sigma}}$ is Morse  with  an index 1 critical point $h_\pm$. By the Morse Lemma and since the differential of $\pi$ in the $I$-direction is nonzero, we can apply the Implicit Function Theorem and choose coordinates $(x,y,z)$ so that ${\Sigma}=\{z=0\}$ and $\pi-\pi(h_\pm)=z-y^2+x^2$. The surface ${\Sigma}$ is cooriented by $\pm\partial z$ and ${\F}_{\pi}$ is directed by $y\partial x + x\partial y$.


As a next step we consider the intersections of these coordinate systems.  First,  choosing sufficiently small neighborhoods  ensures that the neighborhoods of ellliptic and hyperbolic points described above are all disjoint.

If $q$ is a regular point that is in the neighborhood of another regular point $p$ with a coordinate system $(\jel{v,u,}z)$ as above, then we can write $q=(\jel{v_0, u_0},0)$, and construct a new adapted coordinate system: \[(\jel{v',u'},z')=(\jel{v-v_0, u-u_0},z).\] 
 
Let $p=(0, r_0,\vartheta_0)\neq (0,0,0)$ be a point on $\Sigma$ in the neighborhood of $e_\pm$. Then $\pi(p)=\vartheta_0$ and the coordinates \[(\jel{v',u'}z')=(\pm (r-r_0),\vartheta-\vartheta_0, z)\] give an adapted coordinate system around $p$. \marginpar{\jel{here's the problem:  $r-r_0$ should give the $u$ coordinate.}}

Similarly, let $p=(x_0,y_0,0)\neq (0,0,0)$ be a point on ${\Sigma}$ in the neighborhood of $h_\pm$. 
Note that since we are on ${\Sigma}=\{z=0\}$ but in the complement of $(0,0,0)$, at least one of $x_0$ or $y_0$ must be nonzero. Without loss of generality we can assume that  $x_0>0$. In this case the coordinates 
\[(u',v',z')=\big(xy-x_0y_0,(z-x^2+y^2)-(-x_0^2+y_0^2), (\log(x)+2z)-\log(x_0)\big)\] 
are defined in a neighborhood of $x_0$ with $x>0$, and this gives an adapted coordinate system in a neighborhood of $p$.

Finally, using these local models for $\F_{\pit}$ and $\F_{\pit}'$ we can define local maps that take the corresponding coordinate systems to each other. Then we can use a partition of unity to construct a global map $\Psi\colon N \to N'$ from the local ones. Near the elliptic points, the map brings the coordinate systems for the elliptic points to each other, so $\psi$ satisfies conclusion (3). Conclusion (1) is automatically satisfied by the construction. As for conclusion (2), we need to check that $\pi'\circ \psi=\pi$. This is certainly true for the local maps, and the construction of $\psi$ used their convex combinations. In the above change of coordinate systems, the value of $\pi$ was implicit in the system, so we can assume that we only need to take the convex combination of adapted coordinate systems in the neighborhood of regular points. These form a convex set, thus the value of $\psi\circ \pi$ is unchanged while taking their convex combination.

As for the second part, concerning compatible contact structures, let $(S,h)$ be an abstract open book corresponding to $(B,\pi)$. From now on we will assume that $M$ is identified with $M(S,h)$. We briefly recall the Thurston--Winkelnkemper construction \cite{TW} of a contact structure $\widetilde{\xi}=\ker\widetilde{\alpha}$ on $M$ supported by $(B,\pi)$. The construction depends on 
\begin{itemize}
\item[-] a 1-parameter family of 1-forms $(\beta_t)_{t\in [0,1]}$ on the page $S$, such that $d\beta_t$ is an area form on $S$ with total area $2\pi$ and $h_*\beta_0=\beta_1$; and 
\item[-] a sufficiently large constant $\widetilde{C}$. 
\end{itemize}
Then the contact form $\widetilde{\alpha}$ is defined away from $N(B)$ by $\beta_t+\widetilde{C}dt$. In a smaller neighborhood of the binding identified as $B(\varphi) \times D^2(r,\vartheta)$, the contact form $\widetilde{\alpha}$ is given by $2d\varphi+r^2d\vartheta$. In the complement of the two neighborhoods the construction gives an explicit mutual extension of the two 1-forms. 

Let $(S',h')$ be the abstract open book corresponding to $(B',\pi')$, and as before, assume that $M'$ is identified with $M(S',h')$. Take the 1-parameter family of 1-forms  $\widetilde{\beta}'_t=(\Psi\vert_{(S\times\{t\})\cap U})_*\beta_t$ on $(S'\times \{t\})\cap N'$ and choose an area form on $S'$ so that $d\widetilde{\beta}'_t$ has total area less than $2\pi-\varepsilon$ on any closed subset of $(S'\times \{t\})\cap N'$.
Since $\Psi$ respects the monodromies $h$ and $h'$, we have that 
$\widetilde{\beta}_1=h'_*\widetilde{\beta}'_0$ wherever both are defined. Thus we can extend $\widetilde{\beta}'_t$ to an area form $\beta'_t$ on $S'_t$ satisfying the conditions of the Thurston and Winkelnkemper construction, and now a compatible contact form may be defined by a choice of a sufficiently large constant $\widetilde{C}'$. 

Let $C=\max\{\widetilde{C},\widetilde{C}'\}$ and define the contact forms $\alpha$ on $M$ and $\alpha'$ on $M'$ by the Thurston--Winkelnkemper construction using the parameters $\beta_t$ and $C$, and $\beta_t'$ and $C$, respectively. For the corresponding contact structures $\xi=\ker\alpha$ and $\xi'=\ker\alpha'$ we get that $\Psi\vert_N$ is a contactomorphism between $(N,\xi\vert_N)$ and $(N',\xi'\vert_{N'})$, as needed.
\end{proof}
In order to give an explicit model for the open book in $N(\Sigma)$,  the next subsection  constructs a simple open book for a $\Sigma$-bundle over a circle with a prescribed open book foliation on $\Sigma\times \{0\}$.




\subsection{An open book for a surface bundle with prescribed open book foliation on its fibers}\label{sec:egcircle} 
In this section we will show that every circle-free open book foliation $(\F_{\pit}, \pit,H=H_+\cup H_-)$ on a  surface $\Sigma$ is in fact induced by an embedding of $\Sigma$ into an open book.  
%foliation that ``looks like''  an open book foliation is in fact an open book foliation. % \marginpar{\jel{I don't think I agree, as ob implies that the surface is embedded in a fibration.}\vv{Let's discuss!}}
%Let $\Sigma$ be a surface and consider the tuple $\F=(E, \pit,H=H_+\cup H_-)$, where $E$ is a discrete set of points, $\pit\colon \Sigma\!\smallsetminus\! E\to S^1$ is an $S^1$-valued Morse function with only index 1 critical points $H$, and in a $D^2$ neighborhood of each $e\in E$, $\pit$ restricts to $\pm \vartheta$ in polar coordinates $(r,\vartheta)$ on $D^2$. This local model also separates the set of elliptic points $E$ as the union of two subsets $E_+$ and $E_-$. Note that the separation of $H$ into $H_+$ and $H_-$ is part of the defining data, rather than a consequence of $\pit$. The vector $\partial \pit$ co-orients the leaves $\pit^{-1}(t)$ and, because $\Sigma$ is  oriented,   this orients the leaves as well. It is immediate that the foliation induced by  embedding  $\Sigma$ in an open book has these properties. 

As $(\F_{\pit}, \pit, H=H_+\cup H_-)$ is  circle-free, we can construct the dividing curve $\Gamma$ and   see 
that $\pit\vert_\Gamma$ is a covering of $S^1$ of degree $n$, where $n=|E_+|=|E_-|$. Let $\{\Gamma_i\}_{i=1}^k$ be the set of connected components of $\Gamma$ and let $n_i$ be the degree of $\pit\vert_{\Gamma_i}$. Note that $n=\sum_{i=1}^k n_i$. Then we can choose local coordinates $(v,u)$ on $A_i=N(\Gamma_i)$ so that $\pit=n_iv$, $\Gamma=\{u=0\}$, and $\partial u$ directs the level sets $\pit^{-1}(t)$. Define $A=\cup A_i=N(\Gamma)$ and $R_\pm'=R_\pm\!\smallsetminus\! A$. 
 We next construct a characteristic foliation on $\Sigma$ that is also divided by $\Gamma$.

\begin{lemma}[Approximating $\F_{\pit}$ by $\F_{\xi}$]\label{lem:approx}
Let $\Gamma(\F_{\pit})$ be the dividing curve and $R_\pm(\F_{\pit})$ the corresponding positive and negative regions of the open book foliation $(\F_{\pit}, \pit,H=H_+\cup H_-)$. 
Then there is a 1-form $\beta$ that agrees with $d\pit$ away from a small neighborhood of the singular points and $\pm d\beta>0$ on $E_\pm\cup H_\pm$.  The foliation $\F_\beta$ defined by $\beta$ has the same singular points and  is strongly topologically conjugate to $\F_{\pit}$.


Moreover, there is a positive function $g\colon \Sigma\to \R_{>0}$ so that $\beta'=g\beta$ is divided by $\Gamma$, (i.e., $\pm d\beta'>0$ on $R_\pm(\F_{\pit})$ and $\beta\big(T\Gamma(\F_{\pit})\big)>0)$. Furthermore, we may assume that $g<1$ on $A=N\big(\Gamma(\F_{\pit})\big)$. 
\end{lemma} 
\begin{proof}
For the first statement we start with the 1-form $d\pit$ on $\Sigma\!\smallsetminus\! E$ and modify it in the neighborhood of the singular points of $\F_{\pit}$.

Recall that an elliptic point $e\in E_\pm$ has a neighborhood $D^2_\varepsilon(r,\vartheta)$ where $\pit=\pm\vartheta$, so $d\pit=\pm 1$ on $D^2_\varepsilon \!\smallsetminus\!\{e\}$. Define $\beta=\pm\Psi^{\varepsilon}_{\varepsilon/2}r^2d\vartheta$, where $\Psi^{\varepsilon}_{\varepsilon/2}$ is a smooth bump function that equals $1$ for $r<\varepsilon/2$, $0$ for $r>\varepsilon$ and is strictly monotonically decreasing on $[\varepsilon/2,\varepsilon]$. At $e$ we have $\pm d\beta=2r dr\wedge d\vartheta$, which is a positive multiple of a volume form. 

In a neighborhood of a  hyperbolic point $h\in H_\pm$, we can chose local coordinates  so that $\pit=x^2-y^2$. Thus $d\pit=2xdx-2ydy$ and $d^2\pit=0$.  Let $\beta=d\pit\pm \Psi^\varepsilon_{\varepsilon/2} xdy$. Then, as $d\Psi^\varepsilon_{\varepsilon/2}=0$ at $r=0$, we have that $\pm d_h\beta= dx\wedge dy$, a positive multiple of the volume form. 

Extend the 1-form on $\Sigma\setminus N(E\cup H)$ as $d\pit$ to  obtain a 1-form $\beta$ that satisfies the conditions of the first claim. 

Without the assumption $g<1$ on $A$, the second statement is standard in contact geometry. %\marginpar{\vv{I found some sort of reference in John's notes on convex surfaces Thm 2.20, but there the statement is for $X$ and he changes $\omega$.. I will also check Giroux later.}} 
We will recall the proof in our context to see that we can prescribe $g$ to be arbitrarily small where required. Choose a Morse function $h$ on $\Sigma$ whose gradient flow with respect to some metric  directs $\F_\beta$ and that satisfies the following conditions:
% \vv{such a Morse function has been used by Kyle as well, so maybe we don't need to prove its existence} \jel{Is this meant to be a globally defined function?  I think KH only constructs this on a subsurface where existence is clear.} \vv{Yes, this is global, the existence should be clear everywhere too, this is some sort of arclength of the leaves.. Kyle uses it in Example 4.3. He also gives a } 
\begin{itemize} 
\item[-] $\Gamma=h^{-1}(0)$;
\item[-] $A=h^{-1}[-\varepsilon,\varepsilon]$, so that $h=u$;
\item[-] $\partial v$ orients the level sets of $h$. 
\end{itemize}
Such a Morse function exists by Theorem B of \cite{Smale}, and we  use it to define
% https://web.ma.utexas.edu/users/dafr/M392C-2018-MorseTheory/Readings/Smale2.pdf  So we choose local Morse models near H and then Smale promises a global Morse function.  
 $g=h^2+1-2\varepsilon$.  Assuming that $\varepsilon<1/2$, the function $g$ is indeed positive on $\Sigma$, $\beta'(T\Gamma)=g\beta(\partial v)=g\d\pit(\partial v)>0$, and 
\[\pm d\beta'=\pm dg\wedge\beta\pm gd\beta.\]
The second term  on the right vanishes away the singular points and is a positive multiple of a volume form near the singular points. As for the first term, we have $dg=2hdh$.  Recall that the gradient vector field of $h$ directs $\F_\beta$, so $dh\wedge\beta>0$ and the sign of $h$ is $\pm$ in $R_\pm$. 
This proves that $\pm d\beta'>0$ everywhere on $R_\pm$ and as required, $g=h^2+1-2\varepsilon\le 1-\varepsilon<1$ on $A$. 
\end{proof}
%\begin{proof} Sivek Thm 21,
% \vv{, nothing more. we should comment out everything colorfull  after you read it}
%\vv{Justa scetch, but Important to check!}
%\vv{reformulation, please check} A singular foliation $\F=[\beta]$ is \emph{divided} by $\Gamma$ if there exists $\beta'=g\beta$ such that $\pm d\beta'>0$ on $R_\pm$ and $\beta(T\Gamma)>0$. 
%
%\jel{Here's equivalence with definition given in discussion after Thm 3.2: By def, $[\beta']=[g\beta]$.  Define $R^\pm$ as the region where $\pm d\beta'>0$, then $\Gamma$ separates.  Since $\beta'(T\Gamma)>0$, we have that $\F_[\beta]\pitchfork \Gamma$.  Finally, Cartan says $\mathcal{L}_X \omega=\iota_X d\omega+d(\iota_X\omega)$.  The middle term vanishes since $d \omega$ on a surface is $0$.  Thus we substitute $\mathcal{L}_X \omega=d(\iota_X(\omega))=d\beta'$, and we get the required inequalities.  But maybe we also need to specify that $X$ points outward along $\partial R^+$? } \vv{Actually $\beta(T\Gamma)>0$ gives that too. }
%\jel{ Since $X$ is everywhere transverse to $\Gamma$, it must point always out on a fixed component or always in, but it's not clear that this follows from the other properties. }
%An embedded multicurve ? divides a foliation F on ? if ? is transverse to F, ? separates ? into R+ ? R?, and furthermore there exist a volume form ? on ? and a vector field X directing F? such that LX ? is positive on R+ and negative on R? and such that X points outwards along ¶R+.

%\vv{reformulating Sivek Thm 21 to our settings:}
%Suppose that $\F_\xi=[\beta]$, as above, is divided by $\Gamma$. This means that there is a $\beta'=g\beta$ for $g>0$ such that
%$\pm d\beta'>0$ on $R_\pm$ and $\beta'(T\Gamma)>0$. 
%The one form 
%\[\beta'+fdz\] gives a contact structure iff
%\[fd\beta'-df\wedge \beta'>0\]
%Choose $f=\pm 1$ on $R_\pm'$. Then he constructs the rest of $f$ on a neighborhood of $A$ \vv{(his coordinates are as ours, just $(p,s)=(v,u)$ for us)}
%
%\[
%h(v,u)=\exp(-\int_0^u d\beta'(v,t)dt) 
%\]
%\jel{Checked: this is the same orientation of $A$ as we use. Map $(p,s)$ to $(u,v)=(-s,p)$. So I think the upper limit of integration should be $-u$?}
%
%\vv{I know we use $t$ for something else...}
%He sets $f=lh$ such that blaah...
%\end{proof}


We use the functions $f$ from Proposition \ref{prop:Gi} and $g$ from Lemma \ref{lem:approx} to construct both a contact structure and an open book for a $\Sigma$-bundle over  $S^1$. Consider the product $\Sigma\times \R$ with the contact structure defined as the kernel of the 1-form \[\alpha'=\beta'+f dz.\] Let $B'=E\times \R$, where the orientation of $\{e\}\times \R$ is given by $\pm\partial z$ for $e\in E_\pm$. Consider the function \[\pi'=\pit+fz\colon \Sigma\times \R\to S^1,\] %here the sign ``$+$'' stands for the action of $\R$ by translation on $S^1=\R/\mathbb{Z}$. 
where adding $f(x,z)z\in \mathbb{R}$ to $\pit(x,z)$ indicates translation by the image of $fz$ in the quotient $S^1=\mathbb{R}\slash \mathbb{Z}$. 

We would like to glue $\Sigma\times \{0\}$ to $\Sigma\times\{l\}$ for some $l\in\mathbb{N}$ to get an open book and a contact structure for a $\Sigma$-bundle over  $S^1$ . As $f=\pm 1$ on $R_\pm'$, we have $\pi'(x,0)=\pi'(x,l)$ on $R_\pm'$. 
On $A_i=N(\Gamma_i)\cong\Gamma_i\times [-\varepsilon,\varepsilon]$, with coordinates $(v,u)$ chosen as in Lemma \ref{lem:approx}, we have $\pi'((v,u),l)-\pi'((v,u),0)=lf(v,u)$, where $f(v,u)$ is independent of $v$ %=\pit/n_i$ \jel{($\pit=n_i v$, but this is $n:1$ and not invertible.)} 
and monotonically decreases from $1$ to $-1$ in $u$. %along each level set $\pit^{-1}(t)$. 
This means that each level set of $\pi'\vert_{\Sigma\times\{l\}}$ restricted to $A_i$ consists of $n_i$ parallel curves connecting the points $(v,-\varepsilon)$ with $(v+2l/n_i,\varepsilon)$. %, here $u$ parametrises the components $\Gamma_i\cong\R/n_i\mathbb{Z}$ of $\Gamma$. 
When $2l$ is divisible by $n_i$, the endpoints of each component therefore have the same $v$ coordinate, as $v$ parmeterizes $S^1\cong \R/\mathbb{Z}$. And in fact, the curve intersects an arbitrary  $v=c$ segment $\frac{2l}{n_i}\in \mathbb{Z}$ times. 

Set  $l=\lcm\{n_i\}_{i=1}^k$ and define a diffeomorphism
 \[\psi=\prod_{i=1}^k D_{\Gamma_i}^{\frac{2l}{n_i}},\] where $D_{\Gamma_i}$ is the right handed Dehn twist along  $\Gamma_i$.  Let  $M_\psi(\Sigma)=\Sigma\times [0,l]/(\psi(x),0)\sim (x,l)$ be the mapping torus of $\psi$.  Then $\pi'(x,0)=\pi'(\psi(x),l)$ on $S^1$ and $\pi'$ descends as $\pi$ to  $M_\psi(\Sigma)\!\smallsetminus\! B$, where $B=B'\slash\sim$. 

%Set  $l=\lcm\{n_i\}_{i=1}^k$ and consider the mapping torus $M_\psi(\Sigma)=\Sigma\times [0,l]/(x,0)\sim (\psi(x),l)$ of the  diffeomorphism  \[\psi=\prod_{i=1}^k D_{\Gamma_i}^{\frac{2l}{n_i}},\] where $D_{\Gamma_i}$ is the right handed Dehn twist along  $\Gamma_i$. Then $\pi'(x,0)=\pi'(h(x),l)$ on $S^1$ and $\pi'$ descends as $\pi$ to  $M_\psi(\Sigma)\!\smallsetminus\! B$, where $B=B'\slash\sim$. 


Notice, too, that since $f$ depends only on $u$ and the Dehn twists were along the $v$-direction in the $A_i$, the 1-form $\alpha'$ descends  to $M_\psi$ as a 1--form $\alpha$, giving a contact structure $\xi$ on $M_\psi$. 

%what if \Gamma is only isotopic through curve transverse to $\F$

\begin{proposition}[Open book for $(M_\psi,\xi)$]\label{prop:obcyl} Via the construction above, any $\F_{\pit}$ determines an open book decomposition $(B,\pi)$ for $M_\psi$. Moreover, $(B,\pi)$ supports the contact structure $\xi=\ker\alpha$. %defined as the kernel of $\alpha=g\beta+fdz$
\end{proposition} 
Before proving the above proposition, we reformulate what it means for an open book decomposition to support a contact form.

\begin{lemma}\label{lem:ob} Let $B$ be a (positively) transverse  knot in $(M,\xi=\ker\alpha)$ and suppose fibers of the map $\pi\colon M\!\smallsetminus\! B\to S^1$  are Seifert surfaces for $B$. Then the pair $(B,\pi)$ is an open book  supporting the contact form $\alpha$ if and only is $d\pi\wedge d\alpha>0$. \qed
\end{lemma}
%\begin{lemma}\label{lem:ob} Let $B$ be a (positively) transverse  knot in $(M,\xi=\ker\alpha)$ and suppose the map $\pi\colon M\!\smallsetminus\! B\to S^1$  restricts as $\pi=\vartheta$ in a neighborhood $N(B)=B\times D^2(r,\vartheta)$ of $B$. Then the pair $(B,\pi)$ is an open book  supporting the contact form $\alpha$ if and only is $d\pi\wedge d\alpha>0$. \qed\end{lemma}


The proof is straightforward and is left to the reader.
%\begin{proof} \vv{As the proof is trivial, I am not sure we should keep it at the end.}\jel{ agreed }
%With the assumption near $B$, the statements $(B,\pi)$ being an open book decomposition and $d\pi\neq 0$ are equivalent, and $d\pi\neq 0$ also follows from $d\pi\wedge d\alpha>0$, thus in the following we can assume that $d\pi\neq 0$. This means, that we can choose a local coordinate system $(u,v,w)$ so that $\pi=u$ and the level sets of $\pi$ are parametrised by $(v,w)$. By definition we can compute $d\pi\wedge d\alpha(\partial u,\partial v,\partial w)$ as 
%\[d\pi(\partial u)d\alpha(\partial v,\partial w)+d\pi(\partial v)d\alpha(\partial w,\partial u)+d\pi(\partial w)d\alpha(\partial u,\partial v).\]
%As $d\pi=du$, we have:
%\begin{equation*}\label{eq:1}(d\pi\wedge d\alpha)(\partial u,\partial v,\partial w)=d\alpha(\partial v,\partial w)\end{equation*}
%And the left hand side being positive is equivalent to $d\alpha$ being an area form on the level sets of $\pi$, while the right hand side being positive is equivalent to $d\pi\wedge d\alpha$ being a volume form. Thus the above equation proves the statement. 
%
%Which means that $d\alpha$ is an area form on the level sets of $\pi$.
%
%If on the other hand $\alpha$ is supported by $(B,\pi)$, then by definition $d\pi\neq 0$, and we can use the same local coordinates as before, and we again get
%\[(d\pi\wedge d\alpha)(\partial u,\partial v,\partial w)=d\alpha(\partial v,\partial w)>0\]
%This time we deduce that the right hand side is a volume form on $Y$. So the equivalence is proved.  
%\end{proof}





\begin{proof}[Proof of Proposition \ref{prop:obcyl}.]

In a neighborhood of $B$ the function $\pi$ restricts as $\pm(\vartheta+z)$,
 so we see that $\pi^{-1}(t)$ indeed enters $N(B)$ as a Seifert surface. If we evaluate $\alpha$ on $TB=\pm\partial z$ we get $\alpha(\pm\partial z)=1>0$, as needed. 
 

 
For the second step,  by Lemma \ref{lem:ob} it is sufficient to show that $d\pi\wedge d\alpha >0$ on $M_\psi\!\smallsetminus\! B$. Since $\alpha$ is a contact form,  $\alpha\wedge d\alpha>0$, yielding the following:
\[
(\beta'+fdz)\wedge (d\beta'+df\wedge dz)=dz\wedge(\beta'\wedge df+fd\beta')>0.
\]
%\textcolor{green}{\[(g\beta+fdz)\wedge (dg\wedge \beta +gd\beta+df\wedge dz)=dz\wedge(g\beta\wedge df+fdg\wedge\beta+fg d\beta)>0.=\]}
This in turn is equivalent to the condition that 
%\textcolor{green}{\begin{equation*}\label{eq:area} \omega_0=g\beta\wedge df+fdg\wedge\beta+fgd\beta\end{equation*}}
\[
\omega_0=\beta'\wedge df+fd\beta'
\]
 is an area form on $\Sigma$. 

We compute $d\pi \wedge d\alpha$:
%\textcolor{green}{\[(d\pit+zdf+fdz)\wedge(dg\wedge\beta+ gd\beta+df\wedge dz)=dz\wedge(d\pit\wedge df+fdg\wedge\beta+fgd\beta)
%\]}
\[
(d\pit+zdf+fdz)\wedge(d\beta'+df\wedge dz)=dz\wedge(d\pit\wedge df+fd\beta')
\]
Thus we require that %\textcolor{green}{$\omega'=d\pit\wedge df+fdg\wedge\beta+fgd\beta$}
 $\omega'=d\pit\wedge df+fd\beta'$ is an area form on $\Sigma$.  To check this, we compare the given form to the area form $\omega_0$ given by the contact condition and substitute $\beta'=g\beta$:
\[\omega'=\omega_0+(d\pit-g\beta)\wedge df.\]
In the following we will prove that $(d\pit-g\beta)\wedge df\ge 0$, which implies that  $\omega'>0$.
%The difference between the restrictions of $\alpha'\wedge d\alpha$ and $d\pi\wedge d\alpha$ to $T\Sigma$ is:
%\[(d\pit-g\beta)\wedge df\]

On $R_\pm'$ the differential $df$ is 0, thus $\omega'=\omega_0$, so it is indeed an area form. 


On $A$,  $\beta=d\pit$, so we have   
\[(d\pit-g\beta)\wedge df=(1-g)d\pit \wedge df.\]
Recall that on $A$, $f$ depends only on $u$ and is decreasing, while %decreases in $u$ while 
$\pit$ depends only on $v$ and is increasing. %increases in it.  
Thus $d\pit \wedge df$ is an area form, and as $g<1$ on $A$, so is $(1-g)d\pit \wedge df$, as desired. 
\end{proof}


Note that the pages of $(B,\pi)$ are $l$-fold covers of $\Sigma\!\smallsetminus\! E$ via the map from $\pi^{-1}(t) \to \Sigma\!\smallsetminus\! E$ defined by  $(x,z)\mapsto x$. 


\begin{corollary}[Local model]\label{cor:lm}
Suppose that $\Sigma$ is an embedded surface in a 3-manifold $M$ with an open book $(B,\pi)$ that induces an open book foliation $(\F_{\pit}, \pit,H=H_-\cup H_+)$ on $\Sigma$ with no circle leaves. Then $\Sigma$ has a neighborhood $N(\Sigma)\cong \Sigma\times [-\eta,\eta]$ so that $\pi=\pit+fz$, where $f$ is the  function from Proposition \ref{prop:Gi} that is $\pm 1$ on $R_\pm'$ and monotonically increasing in $u$ on $A=N(\Gamma)$.

Moreover, for any 1-form $\beta'$ that is divided by $\Gamma$, and restricts to $A$ as $gd\pit$ (where $g$ is as in Lemma \ref{lem:approx}), there is a contact structure $\xi$ on $M$ compatible with $(B,\pi)$ so that $\xi\vert_{N(\Sigma)}=\beta'+fdz$. \qed
\end{corollary}

This local model for $\Sigma\times [-\eta, \eta]$ is itself a foliated open book which appears as a submanifold of an open book containing the surface $\Sigma$ with the induced open book foliation.


Notice that  the induced open book foliations on the nearby surfaces $\Sigma\times\{z\}$ are strongly topologically conjugate  to $\F_{\pit}$. One can also understand the restrictions of each page $\pi^{-1}(t)$ to $N(\Sigma)$; the pages are surfaces $\pit^{-1}[t-\eta,t+\eta]\cap R_+'$ and $-\left(\pit^{-1}[t-\eta,t+\eta]\cap R_-'\right)$ glued together with a twisted band. If the interval $ [t-\eta,t+\eta]$ contains only regular values of $\pit$, then $\pi^{-1}(t)\cap N(\Sigma)$ is just a union of $|E_+|=|E_-|$ strips; each strip is a rectangle in $N(\Sigma)$ with a pair of its opposite sides  embedded into $\Sigma\times\{-\eta\}$ and $\Sigma\times \{\eta\}$. If $[t-\eta,t+\eta]$ contains a singular value, then one component of  $\pi^{-1}(t)\cap N(\Sigma)$ is a ``cross'', embedded as a saddle surface. See Figure~\ref{fig:layer} \marginpar{\vv{draw figure}
\jel{Figure~\ref{fig:layer} or something else?} \vv{I wanted to draw a nice one near the hyperbolic and the elliptic points too..}}. The intersection $\pi^{-1}(t)\cap N(\Sigma)$ is singular when $t\pm \eta$ is a singular value. 

\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.3]{layer}
\caption{Level set near $A\times [-\eta,\eta]$}\label{fig:layer}
\end{center}
\end{figure}


%\marginpar{redundant?  compare to para before Prop 3.4 and paras before 4.2.} \jel{yes, hidden} From now on, we will use the term \emph{open book foliation} for any tuple $\F=(\pit,E,H=H_+\cup H_-)$ as above. Specifically,  we require only that $\pit$ is an $S^1$-valued Morse function with only index 1 critcal points at $H$ with distinct critical values  and prescribed local models $\pit=\pm \vartheta$ near the elliptic points, regardless of whether it is induced by an embedding into a classical open book or not.  The \emph{reparametriztaion} of the open book foliation $\F$  with the diffeomorphism $g\colon S^1\to S^1$ is the open book foliation $g(\F)=(\pit\circ g,E,H=H_+\cup H_-)$. 

\subsection{Expansion}\label{sec:exp} In order to understand the relationship between Morse and embedded open books, we will modify our local model by introducing cancelling pairs of critical points.  Let  $\Sigma$ be an orientable surface embedded in a $3$-manifold $M$ whose open book structure induces an open book foliation $\F_{\pit}$ on $\Sigma$.  The above corollary provides a local model for a neighborhood $\Sigma\times[-\eta, \eta]\subset M$, which we take as the starting point for the next result.

\begin{proposition}[Expansion]\label{prop:exp} 
Let $(B_e, \pi_e)$ be the embedded foliated open book for  $\Sigma\times [-\eta, \eta]\subset M$ described in Corollary~\ref{cor:lm}. Then there is an $S^1$-valued Morse function $\pi'\colon \Sigma\times [-\eta,\eta]\setminus B \to S^1$ so that the following hold:
\begin{enumerate}
\item for  $\epsilon > \eta$, $\pi'$ is $C^0$-close to $\pi$ and agrees with $\pi$ outside $\Sigma\times[-\varepsilon,\varepsilon]$;
\item for any hyperbolic point $h_\pm\in H_\pm$ of $\F_{\pit}$, the function $\pi'$ has a pair of canceling critical points $p_{h_\pm}^\pm=h_\pm\times \{\pm\varepsilon\}\in\Sigma_\pm=\Sigma\times \{\pm \varepsilon\}$;
\item the index of $p_{h_\pm}^\pm\in \Sigma_\pm$ is $2$ if the signs of $h_\pm$ and $\Sigma_\pm$ agree, and $1$ otherwise; 
\item $\pi'$ has no other critical points;
\item $\nabla \pi'\in T\Sigma_\pm$;
\item $\pi'$ defines an open book foliation $(\F_{\pi'}^\pm, \pi'\vert_{\Sigma_\pm},H\times\{\pm\varepsilon\}=H_+\times\{\pm\varepsilon\}\cup H_-\times\{\pm\varepsilon\})$ on $\Sigma_\pm$ that is strongly topologically conjugate  to $\F_{\pit}$.   
\end{enumerate} \qed
\end{proposition}



%\jel{old version} \begin{proposition}[Expansion]\label{prop:exp} Consider the embedded foliated open book $(B,\pi)=(B_{e\to e}(\Fob),\pi_{e\to e}(\Fob))$ on $\Sigma\times [-\eta,\eta]$ as above. \marginpar{\jel{As in Corollary~\ref{cor:lm}?  I think it's misleading to call this an OB rather than a local neighborhood in an open book}\ vv{This is an embedded FOB, which happens to be in a local neighborhood. But I think the we are not allowed to use the $B_{e\to e}(\Fob),\pi_{e\to e}(\Fob)$ language here, as it now comes later..}} Then there is an $S^1$-valued Morse function $\pi'\colon \Sigma\times [-\eta,\eta]\setminus B \to S^1$ so that:
%\begin{enumerate}
%\item $\pi'$ is $C^0$ close to $\pi$ and agrees with $\pi$ outside $\Sigma\times[-\varepsilon,\varepsilon]$, where $\varepsilon<\eta$;
%\item for any hyperbolic point $h_\pm\in H_\pm$ of $\F_{\pit}$ the function $\pi'$ has a pair of canceling critical points $p_{h_\pm}^\pm=h_\pm\times \{\pm\varepsilon\}\in\Sigma_\pm=\Sigma\times \{\pm \varepsilon\}$;
%\item the index of $p_{h_\pm}^\pm\in \Sigma_\pm$ is $2$ if the sign of $h_\pm$ and $\Sigma_\pm$ agree, and $1$ otherwise;
%\item $\pi'$ has no other critical points;
%\item $\nabla \pi'\in T\Sigma_\pm$;
%\item $\pi'$ defines an open book foliation $\F_{\pi'}^\pm=(\pi'\vert_{\Sigma_\pm},E\times \{\pm\varepsilon\},H\times\{\pm\varepsilon\}=H_+\times\{\pm\varepsilon\}\cup H_-\times\{\pm\varepsilon\})$ on $\Sigma_\pm$ that is topologically conjugate and \vv{$\delta$-isotopic} to $\F_{\pit}$ and is still divided by $\Gamma$. 
%\end{enumerate} \qed
%\end{proposition}






%As a consequence if we glue $T_m^m=T_m^e\cup T_e^m$ together with $(B_m^m,\pi_m^m)=(B_m^e\cup B_e^m,\pi_m^e\cup\pi_e^m)$ to a 3-manifold with a foliated boundary $(M,\F_{\pi_m})$ and a Morse-foliated open book $(B_m,\pi_m)$ we get a 3-manifold $(M'',\F_{\pi_m})$ diffeomorphic to $(M,\F_{\pi_m})$ via $\psi^m_m=\psi_e^m\circ\psi_m^e$, moreover:
%\begin{proposition}[trivial Morse foliated open book]\label{prop:trivM}
%Let $(B_m,\pi_m)$ be a Morse foliated open book for the 3-manifold with foliated boundary $(M,\F_{\pi_m})$. Then the map $\psi_m^m$ gives a diffeomorphism of the Morse foliated open books $(B_m,\pi_m)$ and $(B_m'',\pi_m'')=(B_m\cup B_m^m,\pi_m\cup\pi_m^m)$.
%\end{proposition}
%Using paralell definitions we can state:
%\begin{proposition}[trivial embedded foliated open book]\label{prop:trive}
%\vv{this is not correct, here we need to cancel the critical points..}
%Let $(B_e,\pi_e)$ be an embedded foliated open book for the 3-manifold with foliated boundary $(M,\F_{\pi_e})$. Then the map $\psi_e^e$ gives a diffeomorphism of embedded foliated open books $(B_e,\pi_e)$ and $(B_e'',\pi_e'')=(B_e\cup B_e^e,\pi_e\cup\pi_e^e)$.
%\end{proposition}
%As a consequence of Propositions \ref{prop:trivM} and \ref{prop:trive} any embedded- (or Morse) foliated open book contains $T_e^e$ (or $T_m^m$) and thus $T_m^e$ (or $T_e^m$) together with the corresponding appropriate open book decompositions in the neighborhood of their boundary. 

\begin{proof}[Proof of Proposition \ref{prop:exp}]
Let $z'$ be the interval coordinate and $x$ and $y$ the surface coordinates in the local model for $\Sigma\times [-\eta,\eta]$ as in Corollary ~\ref{cor:lm}. 
For sufficiently small $z'$, the surfaces $\Sigma\times \{z'\}$ have induced open book foliations that are strongly topologically conjugate  to $\F_{\pit}$.

We will modify $\pi$  near the singular points of  $\F_{\pit}$. First reparametrize the $I$ coordinate by $z$, where $z'=z^3+\rho z$ for some $\rho>0$. Note that $z\in [-\zeta,\zeta]$, where $\zeta^3+\rho\zeta=\eta$. Now define a path of functions $\pi_s$ that agrees with $\pi$ outside of a three-ball neighborhood $B_{\varepsilon}^3(h)$ of each hyperbolic point $h\in H_\pm$ and that is defined as follows on $B_{\varepsilon}(h)$:
\[\pi_s=(1-\Psi_{\varepsilon/2}^{\varepsilon}(r))\pi+\Psi_{\varepsilon/2}^{\varepsilon}(r)(\pit+z^3-sz)=\pit+z^3+z(\rho-(s+\rho)\Psi_{\varepsilon/2}^{\varepsilon}(r)).\]
As before,  $\Psi_{\varepsilon/2}^{\varepsilon}$ is a smooth bump function that equals $1$ for $r< \varepsilon/2$ and $0$ for $r>{\varepsilon}$, and here  $r^2=x^2+y^2+z^2$ is the 3-dimensional distance from $h$ in $B_{\varepsilon}^3$.
Clearly $\pi_{-\rho}=\pi$, and we will show that 
\begin{itemize}
\item[-] $\pi_s$ is a regular function for $s<0$; 
\item[-] $\pi_s$ is non-Morse only for $s=0$,
 with an embryonic critical point at each hyperbolic point; and 
 \item[-] for $s>0$, $\pi_s$ is Morse with two cancelling critical points of index 1 and 2 associated to each hyperbolic point $h$. 
 \end{itemize}
 In order to prove the preceding claim, in the following we determine the critical points of $\pi_s$. Away from $D_{\varepsilon}^3(h)$, the function $\pi_s=\pi$ and thus it is regular, while its differential on $D_{\varepsilon}^3(h)$ is
\[d\pi_s=d\pit+\big(3z^2+\rho-(s+\rho)\Psi_{\varepsilon/2}^{\varepsilon}\big)dz-z(s+\rho)d\Psi_{\varepsilon/2}^{\varepsilon}dr\]

For $r>\varepsilon$ the $\Sigma$-component of  $d\pi_s$ equals $d\pit\neq 0$, and thus $d\pi_s\neq 0$.
In the thickened sphere defined by $A=\{\varepsilon/2\le r\le\varepsilon\}$, observe that the coefficients of  $dx$ and  $dy$ in $d\pit$ are $-2x$ and $2y$,  respectively; thus their proportion is $-x:y$. However, in $z(s+\rho)d\Psi_{\varepsilon/2}^{\varepsilon}dr$ the proportion of the coefficients of $dx$ and $dy$ is $x:y$. This means that if in their sum both coefficients are 0, we must have $x=y=0$. Thus the possible critical points of $\pi_s$ in $A$ are all of the form $(0,0,z)$ with $\varepsilon/2\le z \le\varepsilon$. At these points, the $dz$ coordinate of the equation $d\pi_s=0$ simplifies to
\[3z^2+\rho-(s+\rho)\Psi_{\varepsilon/2}^{\varepsilon}-z(s+\rho)d\Psi_{\varepsilon/2}^{\varepsilon}=0\]
On $A$ we have $3z^2\ge \varepsilon^2/4$, while $\vert\rho-(s+\rho)\Psi_{\varepsilon/2}^{\varepsilon}\vert$ can be $<\varepsilon^2/8$ if we choose both $s$ and $\rho$ small. 
As for the third term,
\[-z(s+\rho)d\Psi_{\varepsilon/2}^{\varepsilon}\le\varepsilon/2(s+\rho)K,\] 
where $K=\max_{\varepsilon/4\le r\le\varepsilon/2}\{-d\Psi_{\varepsilon/2}^{\varepsilon}\}>0$. Thus if we choose $|s+\rho|$ sufficiently small we can ensure that this third term is $<\varepsilon^2/8$ and it follows that $d\pi_s$ is nonzero on A.

For $r<\varepsilon/2$ we have 
$d\pi_s=\d\pit+(3z^2-s)dz$. Thus for $\sqrt{\frac{s}3}<\varepsilon/2$,  there are critical points at $z=\pm \sqrt{\frac{s}3}$. 
 
 
In summary, for sufficiently small $\rho>0$ and $|s|$, the function $\pi_s$ is a Morse function for $s\neq 0$. It is regular whenever $s<0$, it has an embryonic critical point at the hyperbolic points $h$, and it has a pair of cancelling index 1 and 2 critical points for each hyperbolic point $h$ on the surfaces $\Sigma\times\{\pm \sqrt{\frac{s}3}\}$.

In the following we will understand the singularities and the leaves of the foliation induced by $\pi_s$ on $\Sigma\times\{z\}$.
Notice that if we restrict $\pi_s$ to $\Sigma\times\{z\}$, then we get a function $\pit+C$ (for $C=z^3-zs$) in $B_{\varepsilon/2}^3$ and $\pit+C'$ (for $C'=z^3+\rho z$) outside $B_{\varepsilon/2}^3$; thus the level sets of $\pit$ agree with the level sets of $\pi_s\vert_{\Sigma\times\{z\}}$ on $B_{\varepsilon/2}^3\cup\Sigma\!\smallsetminus\! B_{\varepsilon}^3 $. From the previous computation we  see that $\pi_s\vert_{\Sigma\times \{z\}}$ has no critical points in $A=\{\varepsilon/2\le r\le\varepsilon\}$. The fibers of $\pi_s(t)$ on $A\cap \Sigma$ connect the level sets $\pit^{-1}(a)$ on $D^2_{\varepsilon/4}$ to the fibers of $\pit(a-(\rho+s)z)$ of $\Sigma\!\smallsetminus\!\cup_h D^2_{\varepsilon/2}$.%\marginpar{\jel{check, original in comments.}}
%The arcs \jel{??} \marginpar{\vv{the arcs of $\pi_s^{-1}(t)$}}on $A$ connect the leaves $\pit^{-1}(a)$ on $D^2_{\varepsilon/4}$ to the leaves of $\pit(a-(\rho+s)z)$ of $\Sigma\!\smallsetminus\!\cup_h D^2_{\varepsilon/2}$. 
This means that if we choose both $|z|$ and $|\rho+s|$ sufficiently small, the foliation induced by
 $\pi_s\vert_{\Sigma\times\{z\}}$ will be strongly topologically conjugate to $\F_{\pit}$.% moreover these changes can be made arbitrarily small, so for example we can achieve that the neighborhoods of the associated positive graphs $G_{++}$ to the level sets of $\pit$ and $\pi_s\vert_{\Sigma\times \{z\}}$ agree. 

Now fix $s>0$  and $\rho>0$ sufficiently small so that the results above hold and let $\pi'=\pi_s$, $\Sigma_\pm=\Sigma\times\{\pm \sqrt{\frac{s}3}\}$. 
\end{proof}

%\subsection{Trivial foliated open book}\label{ssec:triv}


\begin{corollary} The function $\pi'$ from Proposition~\ref{prop:exp} induces a Morse foliated open book on each  component of $M$ cut along $\Sigma_\pm$. 
\end{corollary}

%\jel{ moved trivial open book to to $T_{m\rightarrow m}$ in next section?}

\subsection{Local Models for Morse Foliated Open Books}
The techniques above may be adapted to the case of Morse foliated open books.  We carefully state the result we will rely on in the next section, but leave the  analogous proof to the reader.

Given 3--manifolds $M$ and $M'$ with properly embedded 1--manifolds $B$ and $B'$, respectively, suppose  that  $\pi:M\setminus B\rightarrow S^1$ and $\pi':M'\setminus B'\rightarrow S^1$  are circle-valued Morse functions.  Let $\Sigma\hookrightarrow Y$ and $\Sigma'\hookrightarrow Y'$ be embedded surfaces with induced open book foliations $(\F_{\pit}, \pit,H=H_+\cup H_-)$, $(\F_{\pit}',\pit', H'=H'_+\cup H'_-)$; we require further that any hyperbolic points of these open book foliations coincide with critical points of the corresponding Morse functions on the ambient manifold.  

\begin{proposition}[Morse Neighborhood Theorem]\label{prop:mnbrh} 
If there is a diffeomorphism $\psi\colon \Sigma\to \Sigma'$ that takes the two open book foliations to each other, then  there are neighborhoods $N=N(\Sigma)$ and $N'=N(\Sigma')$ and an extension of $\psi$ to $\Psi\colon N\to N'$ so that 
\begin{enumerate}
\item $\Psi(B)=B'$;
 \item $\pi=\pi'\circ\Psi$;
 \item $\Psi(B\cap N)=B'\cap N'$ and the trivialisation of $N(B)\cap N\cong (B\cap N)\times D^2$ in which $\pi=\vartheta$ maps to the trivialisation of $N(B')\cap N'\cong (B'\cap N')\times D^2$ in which $\pi'=\vartheta$. \qed
 \end{enumerate}

\end{proposition}

Note that we allow $\Sigma$ to embed into $M$ or $M'$  as the boundary; in this case, the neighbohoods are necessarily one-sided.  

%Following the language and notation of Proposition~\ref{prop:exp},  $N(\Sigma)=\Sigma\times [-\varepsilon, \varepsilon]$ has two boundary components printed with $\mathcal{F}_{\pi'}$ and $-\mathcal{F}_{\pi'}$, respectively.  A small perturbation of $\pi'$ may be applied so that paired critical points have distinct critical values, and we retain the same label for the perturbed function.  Then level sets of   $\pi'$ have two possible forms.  For most values of $t\in S^1,( \pi')^{-1}(t)$ is a product of an interval leaf of the original open book foliation with $[-\varepsilon, \varepsilon]$.  Associated to each original hyperbolic point is a $t$-interval separating its images in $\mathcal{F}_{\pi'}$ and $\mathcal{F}_{\pi'}$; each level set associated to a $t$-valued in this interval  is a thickened $X$:  a union of two such rectangular pages glued along a pair of boundary intervals.















==> pfob.tex <==
% !TEX root = FOB_main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\vv{Further Directions}}
\vv{Foliated open books give a new way to study contact structures with boundary that is particularly useful for gluing. As such it turns out to be the right object to define the contact invariant in bordered Floer homology, and we will present this definition together with its comparison to the gluing result of Honda Kazez and Matic in a future paper with Alishahi, F\"oldv\'ari, Hendricks \marginpar{\jel{surnames only is more standard?   I'm starting to
 think we shouldn't have a PFOB section.} \vv{I agree, let's remove it, and start a new paper, but that's gonna be a painful one, as it'll always refer back to this one, and we can just hope, that we set up the terminology right..}} and Ina Petkova \cite{}. Another obvious direction is to amalgamate partial open books with foliated open books. Our last section presents the brief idea of the definition, without going into the details of uniqueness or existence. } 

\subsection{Partial Foliated Open Books}\label{sec:pfob}

We conclude with a brief look at the relationship between partial and foliated open books from an embedded point of view.  
%Previously we constructed  a partial open book from a sorted foliated open book via a hybrid of Morse and abstract techniques: taking the intersection of the  stable and unstable manifolds of boundary critical points as arcs on abstract pages, we used these to define the $(S,P)$ of an abstract partial open book.  However, we could equivalently have identified the partial open book as an embedded submanifold of the original foliated open book; the setwise difference between the two is a neighborhood of the critical submanifolds together with the foliated boundary $\partial M=\Sigma$.  
\vv{ We start with the manifold an example from Sections~ \ref{sec:pobinfob} and \ref{sec:existfob}.  
Consider $\overline{M}$, but shrink $\overline{M}$  slightly, so that $\pi\colon \overline{M}\to[\varepsilon,1-\varepsilon]$, and extend $M'$ with $S_0\times [1-\varepsilon,\varepsilon]$. This modification is just a matter of viewpoint, so that now $\overline{M}$ is actually embedded into $M'$, and its complement is a neighbourhood of $S_0$, and we still have  $\pi\colon M'\to S^1$, whose image on $\overline{M}$ is $[\varepsilon,1-\varepsilon]$. Consider $R\subset \overline{M}\subset M$, then $R$ is foliated by $\{R_t\}_{t\in [\varepsilon,1-\varepsilon]}$, and we extend $R$ to $S_0\times  [1-\varepsilon,\varepsilon]$ by defining $R_t$ for $t\in [1-\varepsilon,\varepsilon]$ as a cornered neighbourhood of $\pit^{-1}(t)$, not intersecting $B$. This new $R'\cong \partial M'\times I$ is foliated by $\{R_t\}_{t\in S^1}$,  and it behaves like a foliated open book from the $\partial M$-side, and as partial open book when looked at the interior of $M'$. Partial foliated open books generalise this idea:
\begin{definition}
An \emph{(abstract) partial foliated open book} is tuple $(\{S_i\}_{i=1}^l, \{h_{i}\}_{i\in I})$, where $I\subset \{0,\dots, l\}$ and
\begin{itemize}
\item[-] $S_i$ are cornered surfaces with boundary $B\cup \alpha_i$;
\item[-] for $i\in I$, $S_i\subset S_{i-1}$ with $\partial S_i\cap \partial S_{i-1}=B$ and 
 $h_{i}$ is an embedding $S_{i}\hookrightarrow S_{i+1}$, again with $\partial h_i(S_i)\cap \partial S_{i+1}=B$;
\item[-] for $i-1 \notin I$ either  $S_{i-1}\xrightarrow[\gamma_{i-1}]{\text{\textbf{cut}}} S_i$ for a properly embedded arc $\gamma_{i-1}$ with endpoints on $\alpha_{i-1}$ or $S_{i-1}\xrightarrow[p_{i-1},q_{i-1}]{\text{\textbf{add}}} S_i$ for $p_{i-1},q_{i-1}\in \alpha_{i-1}$.
\end{itemize}
\end{definition}
As the name suggests, and as the reader can check, both foliated- and partial open books can be recovered from this definition. We will understand the supported contact structures and its existence and uniqueness in a future paper.}
\marginpar{\vv{Help me, is that what we want? Do we want to unclude this at all, or just start our next paper with this example?}} 

%We call such a layer a \emph{partial foliated open book}.  Topologically, \jel{such a} partial foliated open book is a product $\Sigma\times I$, but its open book structure interpolates between partial boundaries and foliated boundaries: on $\Sigma\times \{0\}$, each $R^\pm$ region is a single page, while on the $\Sigma \times \{1\}$ boundary, we recover the original foliation $\F_{\pit}$.    
%
%Here, we described how a partial foliated open book may be removed from a foliated open book to leave behind a partial open books; in fact, a  partial foliated open book may be constructed for any compatible pair, with the property that gluing a partial foliated open book to a partial open book converts it to a foliated open book.  This invites comparison to the layer $T_{e\rightarrow m}$ of Section~\ref{sec:equiv}, as it similarly converts one boundary condition to another while preserving the supporting contact structure.  However, we note that in contrast to shaving a $T_{e\rightarrow m}$ layer from a Morse open book, a partial foliated open book may deformation retract to the boundary of the manifold, but cannot be assumed  contained in a local neighborhood of the boundary.
\marginpar{\jel{I put this in as a joke for you, but we should decide what we really want to say here.}}
\begin{quote}We have drawn a truly remarkable picture of this construction which this paper is too small to contain.\end{quote}





\section{Partial Foliated Open Books}\label{ssec:PFOB}
\jel{Not sure if this belongs in the paper\dots }
\vv{I think we should at least include the definition, and say that that's exactly what we cut off from FOBs to get POBs, and that this is how you can move in between the two.. Maybe just a comment..}

\begin{definition}\footnote{As there is no good notion for embedded partial open books, we will not be able to give an embedded version for partial foliated open books either.}  A  \emph{partial foliated open book} is a tuple
$(\{S_i\}_{i=1}^n, P, h)$, where each $S_i$ and $P$ is a surface with (cornered) boundary $\alpha_i\cup B$; $B$ is constant among all the surfaces; for each $i<n$, $S_{i+1}$ is constructed from $S_i$ by a single $1$-handle addition or saddle resolution; $P\subset S_{n}$ and $h:P\rightarrow S_0$  is a homeomorphism fixing $B$ pointwise.  Furthermore, $\partial P\cap \partial S_i=B$. \end{definition}


Observe that as the name suggests, a partial foliated open book generalises the two existing open book constructions for manifolds with boundary.  If $P=S_{n}$, (then $n$ is necessarily even and) we get an abstract foliated book. On the other hand, if $n=0$, then we have the data of a partial open book.   The definitions and propositions needed to claim that a partial foliated book supports a unique contact structure are %presumably \vv{let's think this through..} 
\marginpar{\vv{I think we can honestly say that the proof works, I wonder if we should add the statements, with short description on how the proof changes}}
similar to those for the purely foliated or partial case, but we will restrict attention to the specific case of a partial foliated open book for $\Sigma\times I$ that is compatible with a given open book foliation $\F=(\pit,E,H=H_+\cup H_-)$ on $\Sigma$ divided by $\Gamma$. We call this the partial foliated open book $I(\Sigma, \mathcal{F},\Gamma)$, and gluing it to either a partial or foliated open book with an appropriate boundary exchanges the boundary type. See Theorem \ref{} and \ref{} \jel{reference propositions where this is (will be) stated precisely.}

\marginpar{\jel{ Define ``compatible" earlier?  This will be useful whenever we just want to use $\Gamma$.}\vv{check}} 

\subsection{Partial open book for $\Sigma\times I$}
\marginpar{\vv{I haven't checked this part as I am not sure we need it for the paper.. but I don't think we can get away with not defining what does it mean for a contact structure to be supported by a PFOB}}
To begin with, we %we briefly describe \jel{do so?} \vv{maybe this should happen earlier in the intro} the construction of a contact manifold with convex boundary from the data of a partial open book and then 
give an explicit embedded description of the partial open book from \cite{HKM2} Example 2 for the $I$-invariant contact structure on $\Sigma \times I$ with a given dividing curve $\Gamma$. As we will use it in the next subsection, we also fix an open book foliation $\F=(\pit,E,H=H_+\cup H_-)$ divided by $\Gamma$, and the embedding will slightly depend on the foliation $\F$ as well.  For convenience, we refrain from collapsing $(\partial S\!\smallsetminus\! \partial P)\times $ to an interval, instead retaining this component as a bigon whose interior is foliated by intervals.   \marginpar{\jel{Do we need to justify why this OK?  The point is simply that in a ``standard" POB, we can gouge out depression along $\Gamma$ and recover this foliated boundary component.}\vv{I would probably introduce POBs as we use it, and comment it there..}}

 \marginpar{\jel{Is this where we can slip in smoothing?}\vv{looks OK to me}}
\vv{For simplicity in the following we assume that $\Gamma$ has only one component. Everything written down works similarly for more components, but the notation is more complicated.} Let $I=[\varepsilon, 1-\varepsilon]$, where $\varepsilon>0$ is sufficiently small 
  so that $\wtpi^{-1}[-\varepsilon, \varepsilon]$ consists only of regular leaves.  Let $P_t=\wtpi^{-1}(t)\times I$ for $t\in [-\varepsilon, \varepsilon]$.  In order to define $S_t$ for $t\in [\varepsilon, \vv{1}-\varepsilon]$, we describe an $s$-dependent singular foliation $\mathcal{G}\vv{_s}$ in a neighborhood of $\big(\Gamma\cup \wtpi^{-1}[-\varepsilon, \varepsilon]\big) \times I$
 %$\big(\Gamma\cup \wtpi^{-1}[-\varepsilon, \varepsilon]\big) \times I$. 
 
 \jel{We first note that elliptic points of opposite signs are paired by appearing as endpoints of $\wtpi^{-1}(0)$, and that the orientation of $\Gamma$ imposes a cyclic ordering on the elliptic points of the same sign.}
 For each  $s\neq \vv{\frac12}$, there are three topologically distinct types of leaves: regular leaves connecting paired elliptic points; regular leaves connecting elliptic points which appear consecutively along $\Gamma$; and singular leaves with triple points on $\wtpi^{-1}(t)\cap \Gamma$ that arise when a pair of leaves of the first two types coincide on a subinterval.  More precisely, we have the following, which is illustrated in Figure~\ref{fig:buildfol}:
 
 \begin{enumerate}
 \item On $\Sigma_s$, for $|\vv{\frac12}-s|<|\vv{\frac12}-t|$, associated to each point of $\wtpi^{-1}(t)\cap \Gamma$ there is a curve which is tangent to but not separated by $\wtpi^{-1}(t)$ at the intersection point and connects paired elliptic points \vv{which ones are paired? the ones at the endpoint of $\pit^{-1}(t)$, or the ones that are paired for $t\in(-\varepsilon,\varepsilon)$ Is this possible to not separate them?}. For $|t|<\varepsilon$, this curve coincides with $\wtpi^{-1}(t)$.   
 
 \item On $\Sigma_s$, for $|\vv{\frac12}-t|<|\vv{\frac12}-s|$ and $s<\vv{\frac12}$, associated to each point of $\wtpi^{-1}(t)\cap \Gamma$ there is a curve which is tangent to  and crosses $\wtpi^{-1}(t)$   at the intersection point and  connects a positive elliptic point with the next negative elliptic point.  \vv{so there is a next, please number them.}\jel{comment above intended to clarify; do you really think life is better with more indices?}
 
  \item On $\Sigma_s$, for $|\vv{\frac12}-t|<|\vv{\frac12}-s|$ and $s>\vv{\frac12}$, associated to each point of $\wtpi^{-1}(t)\cap \Gamma$ there is a curve  which is tangent to  and crosses $\wtpi^{-1}(t)$   at the intersection point and connects a positive elliptic point with the previous negative elliptic point.  

  \item On $\Sigma_s$, for each pair $(s,t)$ where the above quantities are equal, there is a component  with a singular point at $\wtpi^{-1}(t)\cap \Gamma$ formed by taking the union of leaves of the types above and requiring the two halves connecting the same elliptic point to $\wtpi^{-1}(t)\cap \Gamma$ to coincide.
  \end{enumerate}
 


\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.8]{buildfol1}
\caption{ In each figure, the vertical segment represents $\Gamma$, which is oriented upwards. $\mathcal{F}$ is assumed to intersect $\Gamma$ in horizontal line segments, and the value of $s$ increases from left to right.}\label{fig:buildfol}
\end{center}
\end{figure}

\vv{How do you make sure that every point is covered here, so it indeed gives a foliation?}\jel{I could construct something explicitly: foliate squares by intervals and collapse opposite edges to give foliated bigons.  Apply overlapping foliated bigons of both types to each level of $\Sigma\times I$,  aligning the half leaves of the two types to diverge at the triple points, then throwing away the half leaves based on the $s$ coordinate. It is \textit{not} true that exactly the same portion of $\Sigma_s$ is covered for each $s$; this is the point of the leaves $g_{s,s}$ and $g_{s, 1-s}$ below.  Most of $R^\pm$ is not foliated; only a neighborhood of $\Gamma\cup \wtpi^{-1}(0)$ is foliated on each $\Sigma_s$. }
 
Let $\mathcal{G}_s$ denote the foliation parameterized by $t$ on $\Sigma_s$ and let  $g_{s,t}$ denote the leaf of $\mathcal{G}_s$ which is the union of components of $\mathcal{G}_s$ which intersect $\wtpi^{-1}(t) \cap \Gamma$ \vv{I don't understand, is there more of these?}. Observe that on $\Sigma_s$, the leaves $g_{s,s}$ and $g_{s, \vv{1}-s}$ separate $\mathcal{G}_s$ from the unfoliated part \vv{so which part is foliated?} of the surface. 

Let $R^{s,x}\subset \Sigma_s$ be the region bounded by $g_{s,x}$, for $x\in \{t, \vv{1}-t\}$. \vv{Is there an orientation, so we can really say which part you are talking about.} Note that $R^{s,x}$ is homeomorphic to one of $R^\pm$.

\begin{definition}\label{def:productpob} Define $S_t$ to be the following subset of $\Sigma\times I$:
\[ S_t=\bigcup_s g_{s,t} \cup R^{t,t} \cup R^{\vv{1}-t, t}.\]
\end{definition}

\begin{proposition} The pages $P_t$ and $S_t$ of Definition~\ref{def:productpob} define a partial open book for $\Sigma\times I$ which supports the $I$-invariant contact structure divided by $\Gamma$.
\end{proposition}


\begin{proof} The construction described above decomposes  $\Sigma\times I$ into surface, so the proof requires first showing that the decomposition is in fact a partial open book.  It is immediate that each page $P_t$ is a disjoint union of  $\frac{1}{2}|E|$ rectangles, and we argue that each $S_t$ is homeomorphic to a copy of $\Sigma$ cut open along $\wtpi^{-1}(0)$. To see this, observe that for all $t\in [\varepsilon, \vv{1}-\varepsilon$, $\big(S_t\cap \Sigma_t\big) \cup \big(S_t \cap \Sigma_{\vv{1}-t}\big)\cong R^+ \cup R^-$, and these two ``horizontal" components are joined by $\frac{1}{2}|E|$ ``vertical" strips. For $t\notin\{\varepsilon, \vv{\frac12}, \vv{1}-\varepsilon\}$, there are additionally vertical strips extending from the horizontal components to $\Sigma\times\{\varepsilon, \vv{1}-\varepsilon\}$, but these do not change the homeomorphism type of the surface.  Finally, one may check  that $S_\vv{\frac12}$ is similarly homeomorphic to the other $S$ pages. \jel{Actually, haven't done this yet.} By construction, the pages are locally assembled as products, and all pages meet along $B=E\times I$.   

Next, we verify that the partial open book supports the correct contact structure.   For any partial open book, $\Gamma$ is recovered up to isotopy by collapsing the products $\big(\partial P\!\smallsetminus\! \partial S\big)\times I$ and $\big(\partial S\!\smallsetminus\! \partial P\big)\times I$ to intervals and connecting their endpoints.  In the present case, this is equivalent to collapsing $\mathcal G_{\varepsilon}$ and $\mathcal G_{\vv{1}-\varepsilon}$ to curves separating the positive and negative regions of $\Sigma_\varepsilon$ and $\Sigma_{\vv{1}-\varepsilon}$, so that after smoothing, $\Gamma$ divides the original foliations $\mathcal{F}_\varepsilon$ and $\mathcal{F}_{\vv{1}-\varepsilon}$. Letting $\overline{R}^\pm$ denote the positive and negative regions of the convex boundary of $\Sigma\times I$, we have $\overline{R}^+=\big(R^+\times \{\varepsilon\}\big) \cup (R^-\times \{\vv{1}-\varepsilon\}\big)$ and $\overline{R}^-=\big(R^-\times \{\varepsilon\}\big) \cup (R^+\times \{\vv{1}-\varepsilon\}\big)$. \marginpar{signs might be reversed?} 

\jel{I can cut this into two handlebodies to use a Torisu argument for the rest of the contact structure, but is there an easier way to claim $I$-invariance? }
\vv{Well, the construction sorta goes the oposite way, startting from an $I$-invariant contact structure, and then building up the partial open book from a contact cell-decomposition. I think HKM, has this construction somewhere, so we might be able to just cite.}
\end{proof}

Working from the partial open book just constructed, we will soon define a submanifold of $\Sigma\times I$  as the union of  specified subsurfaces $S'_t\subset S_t$. The portion of $\Sigma_s$ included in the submanifold increases monotonically with $s$ and includes all of $\Sigma_{\vv{1}-\varepsilon}$, so it follows immediately that the object constructed is homeomorphic to $\Sigma\times I$.  In fact, we will show that the submanifold is a partial foliated open book with pages $S'_t$ and $P'_t=P_t$.  As motivation for the somewhat involved construction to come, we note that such ``product partial foliated open books" allow us to transform partial open books to foliated ones, and vice versa.

\begin{theorem} Given any foliated open book $(M, \xi, \mathcal{F})$, after possibly stabilising we may decompose the original object as a partial open book for $(M, \xi, \Gamma)$ together with a product partial foliated open book. Given any partial open book, we may attach  a product partial foliated open book to get a foliated open book. 
\end{theorem}

\subsection{Partial foliated open book for $(\Sigma, \mathcal{F})\times I$.}\label{sec:prodpfob}
\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.8]{buildfol3}
\caption{ The shaded regions of each $\Sigma_s$ indicate the pages of the PFOB for $\Sigma\times I$.  }\label{fig:buildfol}
\end{center}
\end{figure}



\begin{definition}\label{def:productpfob} The PFOB for $\Sigma\times I$ is the subset of $\Sigma \times I$ that contains $P\times [-\varepsilon, \varepsilon]$ and the pages $S'_t$ defined as follows: 


When $\varepsilon<t<\vv{\frac12}$, the intersection of $S'_t$ and $\Sigma_s$ is defined by the following cases:
\begin{itemize}
\item for $t<s$, set $S'_t\cap \Sigma_s=\emptyset$
\item for $t=s$,  set $S'_t\cap \Sigma_t=S_t\cap \Sigma_t \cap \wtpi^{-1}[\varepsilon, t] \cap R^-$
\item for $s<t<\vv{1}-s$,  set $S'_t\cap \Sigma_s=S_t\cap \Sigma_s  \cap R^-$
\item for $s<t<\vv{1}-s$,  set $S'_t\cap \Sigma_s=\big(S_t\cap \Sigma_s  \cap R^-\big)\cup\big(S_t\cap \Sigma_s  \cap R^+ \cap \wtpi^{-1}[\varepsilon, \vv{1}-t]\big)$
\item for $t>\vv{1}-s$, set $S'_t\cap \Sigma_s=S_t\cap \Sigma_s$
\end{itemize}

When $\vv{1}-\varepsilon> t>\vv{\frac12}$,  the intersection of $S'_t$ and $\Sigma_s$ is defined by the following cases:

\begin{itemize}
\item for $\vv{1}-t<s$, $S'_{\vv{1}-t}\cap \Sigma_s=\emptyset$
\item for $\vv{1}-t=s$,  $S'_{\vv{1}-t}\cap \Sigma_t=S_{\vv{1}-t}\cap \Sigma_t \cap \wtpi^{-1}[\vv{1}-t, \vv{1}-\varepsilon] \cap R^+$
\item for $\vv{1}-t<s<t$, $S'_{\vv{1}-t}\cap \Sigma_s=S_{\vv{1}-t}\cap \Sigma_s \cap R^+$
\item for $\vv{1}-t=s$, $S'_{\vv{1}-t}\cap \Sigma_t=\big(S_{\vv{1}-t}\cap \Sigma_s\cap R^+\big)\cup \big(S_{\vv{1}-t}\cap \Sigma_s\cap R^-\cap \wtpi^{-1}[\varepsilon, \vv{1}-t]\big)$
\item for $s<\vv{1}-t$, $S'_{\vv{1}-t}\cap \Sigma_s=S_{\vv{1}-t}\cap \Sigma_s$
\end{itemize}

When $s=t=\vv{\frac12}$, the inequalities in either list above collapse to three conditions which define $S'_\pi$.

For $-\varepsilon<t<\varepsilon$, it is straightforward to describe the entire page:

\begin{itemize}
\item $S'_0=S_0$ 
\item for $0<t<\varepsilon$,  $S'_t\cap R^-=S_t\cap R^-$ and $S'_t\cap R^+=S_t\cap R^+\cap \{0\leq s\leq t\}$
\item for $\vv{1}-\varepsilon<t <\vv{1}$,  $S'_t\cap R^+=S_t\cap R^+$ and $S'_t\cap R^-=S_t\cap R^-\cap \{0\leq s\leq \vv{1}-t\}$

\end{itemize}





Equivalently, letting $\Sigma'_s$ be the subset of $\Sigma_s$ included in the PFOB, we have

\[\Sigma'_s=\big(S_{[0, s]}\cap \Sigma_s \cap g^{-1}[0, s] \cap R^-\big) \cup \big(  S_{[\vv{1}-s, \vv{1}]} \cap \Sigma_s\cap g^{-1}[\vv{1}-s, \vv{1}]\cap R^+\big).\]

Here, $S_{[x,y]}=\bigcup_{t\in [x,y]} S_t$.  
\end{definition}
\vv{What is $g$?}


\jel{somethign about supporting $I$ invariant contact structure?  Old irrelevant lemma commented out.}

\begin{proposition}\label{prop:fpluspf} Suppose that $\mathcal{F}$ is an $S^1$ Morse foliation on $\Sigma=\partial M$, and suppose that $(S,P,h)$ \marginpar{\jel{not nice to mix abstract and embedded objects in one prop...} \vv{It happens, because there is no nonabstract POB, we can probably rephrase the whole statement to an abstract one.}} is a partial open book with the property that $\Gamma$ divides $\mathcal{F}$.  Then one may glue a product partial foliated open book for $(\Sigma, \mathcal{F})$ to along $\Sigma\times \{\vv{1}-\varepsilon\}$ to $M(S,P, h)$ to get a foliated open book $(B, \pi, \mathcal{F})$ compatible with the original $\xi$.
\end{proposition}

Philosophically, the feature distinguishing partial and foliated open books is whether the changes in the topology of the pages happen at just two $t$ values or at many; the product partial foliated open book interpolates between these two cases.  

\begin{proof} We first observe that the gluing makes sense: construct the abstract partial open book from the given data, but do not collapse the foliated bigons to intervals.  Instead, identify $\partial M(S, P, h)$ pagewise with $\wtpi^{-1}(t)\cap \Sigma_{\vv{1}-\varepsilon}$ on the product  partial foliated open book.  We claim that the result is a foliated open book for the original manifold.

 Each original $R^\pm$ on $\Sigma=\partial M$ is exactly the setwise difference between $S$ and the subpages $P$ and $h(P)$, and the product partial foliated open book was constructed so that $S$ is  built up from $P$ (respectively, $h(P)$) via sequence of handle additions, one corresponding to each hyperbolic point in $R^+$ (respectively, $R^-$) as $t$ increases.  Thus the result is an $S^1$-family of pages identified along $B$ whose topology changes by a single $1$-handle addition or saddle resolution at each $t$-value corresponding to a hyperbolic point on the foliated boundary.  Equivalently, there is a \jel{smooth} map from $M\!\smallsetminus\! B\rightarrow S^1$ with only isolated critical points, each located on $\partial M$, so \jel{we may perturb this to an $S^1$-valued Morse function on the complement of the binding.} 
 

Since both the original and new boundary surfaces are divided by $\Gamma$, we may isotope the contact structures in a neighborhood of the gluing surface to agree. Furthermore, the product partial foliated open book supported an $I$-invariant contact structure, so the contact structure supported by the new glued manifold is contactomorphic to the contact structure supported on the original partial open book, as desired.  \vv{We have to clean this up a bit}
\end{proof}

In fact, Proposition~\ref{prop:fpluspf} is the key ingredient in proving that every contact manifold whose boundary has an $S^1$-Morse foliation admits a compatible foliated open book.

\begin{proof}[Proof of Theorem~\ref{thm:exist1}] Given $(M, \xi, \mathcal{F})$, choose a partial open book with $\Gamma$ dividing $\mathcal{F}$.  Then apply Proposition~\ref{prop:fpluspf}.
\end{proof}


\begin{example} \jel{Explain the relationship between 2 PFOBs compatible with the same POB?  (i.e., same $\Gamma$ but different $\mathcal{F}$).  The answer is that we have two PFOBs for $\Sigma\times I$ glued along their P sides to give a new FOB for $\Sigma \times I$.  }
\end{example}

\begin{question} Are there local moves between $(\mathcal{F}_i, f_i)$ $i=1,2$ for the same $\Gamma$?
\end{question}




==> pobOLD.tex <==



\section{Relation to Partial Open Books}
The main tool in proving existence and ``Giroux correspondence'' for foliated open books relies on their deep connection 
to partial open books. This connection is established with an interpolating piece, called partial foliated open book, for a product contact structure. In subsection  \ref{ssec:PFOB} we define partial foliated open books in general, and after giving an explicit description of the partial open book for an $I$ invariant contact structure with a given dividing curve in subsection \ref{sec:prodpfob}, we cut it in half in subsection \ref{} to obtain a partial foliated open book for given foliation $\F$. We will call this partial foliated open book $I(\Sigma, \mathcal{F},\Gamma)$, and it will serve as an interpolating piece between partial open books and foliated open books. Gluing this interpolating piece to a partial open book (see Thm \ref{}) immediately provides a proof for Theorem \ref{}. Later in subsection \ref{} we prove that after possible stabilisation any foliated open book arises in the above form, and we use this statement to prove theorem \ref{}.

\subsection{Partial Foliated Open Books}\label{ssec:PFOB}


\begin{definition}\footnote{As there is no good notion for embedded partial open books, we will not be able to give an embedded version for partial foliated open books either.}  A  \emph{partial foliated open book} is a tuple
$(\{S_i\}_{i=1}^n, P, h)$, where each $S_i$ and $P$ is a surface with (cornered) boundary $\alpha_i\cup B$; $B$ is constant among all the surfaces; for each $i<n$, $S_{i+1}$ is constructed from $S_i$ by a single $1$-handle addition or saddle resolution; $P\subset S_{n}$ and $h:P\rightarrow S_0$  is a homeomorphism fixing $B$ pointwise.  Furthermore, $\partial P\cap \partial S_i=B$. \end{definition}


Observe that as the name suggests, a partial foliated open book generalises the two existing open book constructions for manifolds with boundary.  If $P=S_{n}$, (then $n$ is necessarily even and) we get an abstract foliated book. On the other hand, if $n=0$, then we have the data of a partial open book.   The definitions and propositions needed to claim that a partial foliated book supports a unique contact structure are %presumably \vv{let's think this through..} 
\marginpar{\vv{I think we can honestly say that the proof works, I wonder if we should add the statements, with short description on how the proof changes}}
similar to those for the purely foliated or partial case, but we will restrict attention to the specific case of a partial foliated open book for $\Sigma\times I$ that is compatible with a given open book foliation $\F=(\pit,E,H=H_+\cup H_-)$ on $\Sigma$ divided by $\Gamma$. We call this the partial foliated open book $I(\Sigma, \mathcal{F},\Gamma)$, and gluing it to either a partial or foliated open book with an appropriate boundary exchanges the boundary type. See Theorem \ref{} and \ref{} \jel{reference propositions where this is (will be) stated precisely.}

\marginpar{\jel{ Define ``compatible" earlier?  This will be useful whenever we just want to use $\Gamma$.}\vv{check}} 

\subsection{Partial open book for $\Sigma\times I$}
\marginpar{\vv{I haven't checked this part as I am not sure we need it for the paper.. but I don't think we can get away with not defining what does it mean for a contact structure to be supported by a PFOB}}
To begin with, we %we briefly describe \jel{do so?} \vv{maybe this should happen earlier in the intro} the construction of a contact manifold with convex boundary from the data of a partial open book and then 
give an explicit embedded description of the partial open book from \cite{HKM2} Example 2 for the $I$-invariant contact structure on $\Sigma \times I$ with a given dividing curve $\Gamma$. As we will use it in the next subsection, we also fix an open book foliation $\F=(\pit,E,H=H_+\cup H_-)$ divided by $\Gamma$, and the embedding will slightly depend on the foliation $\F$ as well.  For convenience, we refrain from collapsing $(\partial S\!\smallsetminus\! \partial P)\times $ to an interval, instead retaining this component as a bigon whose interior is foliated by intervals.   \marginpar{\jel{Do we need to justify why this OK?  The point is simply that in a ``standard" POB, we can gouge out depression along $\Gamma$ and recover this foliated boundary component.}\vv{I would probably introduce POBs as we use it, and comment it there..}}

 \marginpar{\jel{Is this where we can slip in smoothing?}\vv{looks OK to me}}
\vv{For simplicity in the following we assume that $\Gamma$ has only one component. Everything written down works similarly for more components, but the notation is more complicated.} Let $I=[\varepsilon, 1-\varepsilon]$, where $\varepsilon>0$ is sufficiently small 
  so that $\wtpi^{-1}[-\varepsilon, \varepsilon]$ consists only of regular leaves.  Let $P_t=\wtpi^{-1}(t)\times I$ for $t\in [-\varepsilon, \varepsilon]$.  In order to define $S_t$ for $t\in [\varepsilon, \vv{1}-\varepsilon]$, we describe an $s$-dependent singular foliation $\mathcal{G}\vv{_s}$ in a neighborhood of $\big(\Gamma\cup \wtpi^{-1}[-\varepsilon, \varepsilon]\big) \times I$
 %$\big(\Gamma\cup \wtpi^{-1}[-\varepsilon, \varepsilon]\big) \times I$. 
 
 \jel{We first note that elliptic points of opposite signs are paired by appearing as endpoints of $\wtpi^{-1}(0)$, and that the orientation of $\Gamma$ imposes a cyclic ordering on the elliptic points of the same sign.}
 For each  $s\neq \vv{\frac12}$, there are three topologically distinct types of leaves: regular leaves connecting paired elliptic points; regular leaves connecting elliptic points which appear consecutively along $\Gamma$; and singular leaves with triple points on $\wtpi^{-1}(t)\cap \Gamma$ that arise when a pair of leaves of the first two types coincide on a subinterval.  More precisely, we have the following, which is illustrated in Figure~\ref{fig:buildfol}:
 
 \begin{enumerate}
 \item On $\Sigma_s$, for $|\vv{\frac12}-s|<|\vv{\frac12}-t|$, associated to each point of $\wtpi^{-1}(t)\cap \Gamma$ there is a curve which is tangent to but not separated by $\wtpi^{-1}(t)$ at the intersection point and connects paired elliptic points \vv{which ones are paired? the ones at the endpoint of $\pit^{-1}(t)$, or the ones that are paired for $t\in(-\varepsilon,\varepsilon)$ Is this possible to not separate them?}. For $|t|<\varepsilon$, this curve coincides with $\wtpi^{-1}(t)$.   
 
 \item On $\Sigma_s$, for $|\vv{\frac12}-t|<|\vv{\frac12}-s|$ and $s<\vv{\frac12}$, associated to each point of $\wtpi^{-1}(t)\cap \Gamma$ there is a curve which is tangent to  and crosses $\wtpi^{-1}(t)$   at the intersection point and  connects a positive elliptic point with the next negative elliptic point.  \vv{so there is a next, please number them.}\jel{comment above intended to clarify; do you really think life is better with more indices?}
 
  \item On $\Sigma_s$, for $|\vv{\frac12}-t|<|\vv{\frac12}-s|$ and $s>\vv{\frac12}$, associated to each point of $\wtpi^{-1}(t)\cap \Gamma$ there is a curve  which is tangent to  and crosses $\wtpi^{-1}(t)$   at the intersection point and connects a positive elliptic point with the previous negative elliptic point.  

  \item On $\Sigma_s$, for each pair $(s,t)$ where the above quantities are equal, there is a component  with a singular point at $\wtpi^{-1}(t)\cap \Gamma$ formed by taking the union of leaves of the types above and requiring the two halves connecting the same elliptic point to $\wtpi^{-1}(t)\cap \Gamma$ to coincide.
  \end{enumerate}
 


\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.8]{buildfol1}
\caption{ In each figure, the vertical segment represents $\Gamma$, which is oriented upwards. $\mathcal{F}$ is assumed to intersect $\Gamma$ in horizontal line segments, and the value of $s$ increases from left to right.}\label{fig:buildfol}
\end{center}
\end{figure}

\vv{How do you make sure that every point is covered here, so it indeed gives a foliation?}\jel{I could construct something explicitly: foliate squares by intervals and collapse opposite edges to give foliated bigons.  Apply overlapping foliated bigons of both types to each level of $\Sigma\times I$,  aligning the half leaves of the two types to diverge at the triple points, then throwing away the half leaves based on the $s$ coordinate. It is \textit{not} true that exactly the same portion of $\Sigma_s$ is covered for each $s$; this is the point of the leaves $g_{s,s}$ and $g_{s, 1-s}$ below.  Most of $R^\pm$ is not foliated; only a neighborhood of $\Gamma\cup \wtpi^{-1}(0)$ is foliated on each $\Sigma_s$. }
 
Let $\mathcal{G}_s$ denote the foliation parameterized by $t$ on $\Sigma_s$ and let  $g_{s,t}$ denote the leaf of $\mathcal{G}_s$ which is the union of components of $\mathcal{G}_s$ which intersect $\wtpi^{-1}(t) \cap \Gamma$ \vv{I don't understand, is there more of these?}. Observe that on $\Sigma_s$, the leaves $g_{s,s}$ and $g_{s, \vv{1}-s}$ separate $\mathcal{G}_s$ from the unfoliated part \vv{so which part is foliated?} of the surface. 

Let $R^{s,x}\subset \Sigma_s$ be the region bounded by $g_{s,x}$, for $x\in \{t, \vv{1}-t\}$. \vv{Is there an orientation, so we can really say which part you are talking about.} Note that $R^{s,x}$ is homeomorphic to one of $R^\pm$.

\begin{definition}\label{def:productpob} Define $S_t$ to be the following subset of $\Sigma\times I$:
\[ S_t=\bigcup_s g_{s,t} \cup R^{t,t} \cup R^{\vv{1}-t, t}.\]
\end{definition}

\begin{proposition} The pages $P_t$ and $S_t$ of Definition~\ref{def:productpob} define a partial open book for $\Sigma\times I$ which supports the $I$-invariant contact structure divided by $\Gamma$.
\end{proposition}


\begin{proof} The construction described above decomposes  $\Sigma\times I$ into surface, so the proof requires first showing that the decomposition is in fact a partial open book.  It is immediate that each page $P_t$ is a disjoint union of  $\frac{1}{2}|E|$ rectangles, and we argue that each $S_t$ is homeomorphic to a copy of $\Sigma$ cut open along $\wtpi^{-1}(0)$. To see this, observe that for all $t\in [\varepsilon, \vv{1}-\varepsilon$, $\big(S_t\cap \Sigma_t\big) \cup \big(S_t \cap \Sigma_{\vv{1}-t}\big)\cong R^+ \cup R^-$, and these two ``horizontal" components are joined by $\frac{1}{2}|E|$ ``vertical" strips. For $t\notin\{\varepsilon, \vv{\frac12}, \vv{1}-\varepsilon\}$, there are additionally vertical strips extending from the horizontal components to $\Sigma\times\{\varepsilon, \vv{1}-\varepsilon\}$, but these do not change the homeomorphism type of the surface.  Finally, one may check  that $S_\vv{\frac12}$ is similarly homeomorphic to the other $S$ pages. \jel{Actually, haven't done this yet.} By construction, the pages are locally assembled as products, and all pages meet along $B=E\times I$.   

Next, we verify that the partial open book supports the correct contact structure.   For any partial open book, $\Gamma$ is recovered up to isotopy by collapsing the products $\big(\partial P\!\smallsetminus\! \partial S\big)\times I$ and $\big(\partial S\!\smallsetminus\! \partial P\big)\times I$ to intervals and connecting their endpoints.  In the present case, this is equivalent to collapsing $\mathcal G_{\varepsilon}$ and $\mathcal G_{\vv{1}-\varepsilon}$ to curves separating the positive and negative regions of $\Sigma_\varepsilon$ and $\Sigma_{\vv{1}-\varepsilon}$, so that after smoothing, $\Gamma$ divides the original foliations $\mathcal{F}_\varepsilon$ and $\mathcal{F}_{\vv{1}-\varepsilon}$. Letting $\overline{R}^\pm$ denote the positive and negative regions of the convex boundary of $\Sigma\times I$, we have $\overline{R}^+=\big(R^+\times \{\varepsilon\}\big) \cup (R^-\times \{\vv{1}-\varepsilon\}\big)$ and $\overline{R}^-=\big(R^-\times \{\varepsilon\}\big) \cup (R^+\times \{\vv{1}-\varepsilon\}\big)$. \marginpar{signs might be reversed?} 

\jel{I can cut this into two handlebodies to use a Torisu argument for the rest of the contact structure, but is there an easier way to claim $I$-invariance? }
\vv{Well, the construction sorta goes the oposite way, startting from an $I$-invariant contact structure, and then building up the partial open book from a contact cell-decomposition. I think HKM, has this construction somewhere, so we might be able to just cite.}
\end{proof}

Working from the partial open book just constructed, we will soon define a submanifold of $\Sigma\times I$  as the union of  specified subsurfaces $S'_t\subset S_t$. The portion of $\Sigma_s$ included in the submanifold increases monotonically with $s$ and includes all of $\Sigma_{\vv{1}-\varepsilon}$, so it follows immediately that the object constructed is homeomorphic to $\Sigma\times I$.  In fact, we will show that the submanifold is a partial foliated open book with pages $S'_t$ and $P'_t=P_t$.  As motivation for the somewhat involved construction to come, we note that such ``product partial foliated open books" allow us to transform partial open books to foliated ones, and vice versa.

\begin{theorem} Given any foliated open book $(M, \xi, \mathcal{F})$, after possibly stabilising we may decompose the original object as a partial open book for $(M, \xi, \Gamma)$ together with a product partial foliated open book. Given any partial open book, we may attach  a product partial foliated open book to get a foliated open book. 
\end{theorem}

\subsection{Partial foliated open book for $(\Sigma, \mathcal{F})\times I$.}\label{sec:prodpfob}
\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.8]{buildfol3}
\caption{ The shaded regions of each $\Sigma_s$ indicate the pages of the PFOB for $\Sigma\times I$.  }\label{fig:buildfol}
\end{center}
\end{figure}



\begin{definition}\label{def:productpfob} The PFOB for $\Sigma\times I$ is the subset of $\Sigma \times I$ that contains $P\times [-\varepsilon, \varepsilon]$ and the pages $S'_t$ defined as follows: 


When $\varepsilon<t<\vv{\frac12}$, the intersection of $S'_t$ and $\Sigma_s$ is defined by the following cases:
\begin{itemize}
\item for $t<s$, set $S'_t\cap \Sigma_s=\emptyset$
\item for $t=s$,  set $S'_t\cap \Sigma_t=S_t\cap \Sigma_t \cap \wtpi^{-1}[\varepsilon, t] \cap R^-$
\item for $s<t<\vv{1}-s$,  set $S'_t\cap \Sigma_s=S_t\cap \Sigma_s  \cap R^-$
\item for $s<t<\vv{1}-s$,  set $S'_t\cap \Sigma_s=\big(S_t\cap \Sigma_s  \cap R^-\big)\cup\big(S_t\cap \Sigma_s  \cap R^+ \cap \wtpi^{-1}[\varepsilon, \vv{1}-t]\big)$
\item for $t>\vv{1}-s$, set $S'_t\cap \Sigma_s=S_t\cap \Sigma_s$
\end{itemize}

When $\vv{1}-\varepsilon> t>\vv{\frac12}$,  the intersection of $S'_t$ and $\Sigma_s$ is defined by the following cases:

\begin{itemize}
\item for $\vv{1}-t<s$, $S'_{\vv{1}-t}\cap \Sigma_s=\emptyset$
\item for $\vv{1}-t=s$,  $S'_{\vv{1}-t}\cap \Sigma_t=S_{\vv{1}-t}\cap \Sigma_t \cap \wtpi^{-1}[\vv{1}-t, \vv{1}-\varepsilon] \cap R^+$
\item for $\vv{1}-t<s<t$, $S'_{\vv{1}-t}\cap \Sigma_s=S_{\vv{1}-t}\cap \Sigma_s \cap R^+$
\item for $\vv{1}-t=s$, $S'_{\vv{1}-t}\cap \Sigma_t=\big(S_{\vv{1}-t}\cap \Sigma_s\cap R^+\big)\cup \big(S_{\vv{1}-t}\cap \Sigma_s\cap R^-\cap \wtpi^{-1}[\varepsilon, \vv{1}-t]\big)$
\item for $s<\vv{1}-t$, $S'_{\vv{1}-t}\cap \Sigma_s=S_{\vv{1}-t}\cap \Sigma_s$
\end{itemize}

When $s=t=\vv{\frac12}$, the inequalities in either list above collapse to three conditions which define $S'_\pi$.

For $-\varepsilon<t<\varepsilon$, it is straightforward to describe the entire page:

\begin{itemize}
\item $S'_0=S_0$ 
\item for $0<t<\varepsilon$,  $S'_t\cap R^-=S_t\cap R^-$ and $S'_t\cap R^+=S_t\cap R^+\cap \{0\leq s\leq t\}$
\item for $\vv{1}-\varepsilon<t <\vv{1}$,  $S'_t\cap R^+=S_t\cap R^+$ and $S'_t\cap R^-=S_t\cap R^-\cap \{0\leq s\leq \vv{1}-t\}$

\end{itemize}





Equivalently, letting $\Sigma'_s$ be the subset of $\Sigma_s$ included in the PFOB, we have

\[\Sigma'_s=\big(S_{[0, s]}\cap \Sigma_s \cap g^{-1}[0, s] \cap R^-\big) \cup \big(  S_{[\vv{1}-s, \vv{1}]} \cap \Sigma_s\cap g^{-1}[\vv{1}-s, \vv{1}]\cap R^+\big).\]

Here, $S_{[x,y]}=\bigcup_{t\in [x,y]} S_t$.  
\end{definition}
\vv{What is $g$?}

%\begin{lemma} For all $t$, $\partial S'_t\!\smallsetminus\! \partial S_t$ is Legendrian in $\Sigma\times I$ with the supported $I$-invariant contact structure.  Thus, the foliation on the new boundary of the product partial foliated open book is characteristic.  \vv{What does this mean? Why do we need this?}\jel{Old, when whe}
%\end{lemma}


%\begin{proof} The contact structure supported by the partial open book is invariant under translation in $s$-direction, and $\Gamma\times \{s\}$ divides $\mathcal{F}_s$ on each convex $\Sigma_s$.  Applying Giroux \jel{cite} once again, we may assume that $\mathcal{F}\times s$ is the characteristic foliation \vv{Isn't $\F$ an $S^1$-Morse foliation, this is where we have to be careful about coincidence vs. conjugacy?} on each surface  $\Sigma\times s$. For $t\in [\varepsilon, \vv{1}-\varepsilon]$, each component of $\partial S'_t\!\smallsetminus\! \partial S_t$ is a concatenation of horizontal and vertical segments.  The horizontal curves are subsets of the characteristic foliations on $\Sigma_t$ and $\Sigma_{\vv{1}-t}$, and hence are Legendrian. Each of these curves has an endpoint on $B$  and the free endpoints are connected pairwise by a vertical segment $\wtpi^{-1}(t)\cap \Gamma\times I'$, where $I'\subset I$ is the interval betwee the two horizontal components.  Since $\Gamma$ divides each $\Sigma_s$, we may suppose that $\alpha (ds)=0$ along $\Gamma$, so the vertical segments are also Legendrian.  \jel{Rigorously, why?} \vv{Exactly because of this, the definition of $\Gamma$ is that $\partial s\in \xi$. We just have to define what we mean by $I$-invariant contact structure for a given dividing curve, but that should be it.}
%Projecting this curve in the $s$-direction yields a copy of $\wtpi^{-1}(t)$, and this projection is injective except along the vertical segment.  \end{proof}

\jel{somethign about supporting $I$ invariant contact structure?  Old irrelevant lemma commented out.}

\begin{proposition}\label{prop:fpluspf} Suppose that $\mathcal{F}$ is an $S^1$ Morse foliation on $\Sigma=\partial M$, and suppose that $(S,P,h)$ \marginpar{\jel{not nice to mix abstract and embedded objects in one prop...} \vv{It happens, because there is no nonabstract POB, we can probably rephrase the whole statement to an abstract one.}} is a partial open book with the property that $\Gamma$ divides $\mathcal{F}$.  Then one may glue a product partial foliated open book for $(\Sigma, \mathcal{F})$ to along $\Sigma\times \{\vv{1}-\varepsilon\}$ to $M(S,P, h)$ to get a foliated open book $(B, \pi, \mathcal{F})$ compatible with the original $\xi$.
\end{proposition}

Philosophically, the feature distinguishing partial and foliated open books is whether the changes in the topology of the pages happen at just two $t$ values or at many; the product partial foliated open book interpolates between these two cases.  

\begin{proof} We first observe that the gluing makes sense: construct the abstract partial open book from the given data, but do not collapse the foliated bigons to intervals.  Instead, identify $\partial M(S, P, h)$ pagewise with $\wtpi^{-1}(t)\cap \Sigma_{\vv{1}-\varepsilon}$ on the product  partial foliated open book.  We claim that the result is a foliated open book for the original manifold.

 Each original $R^\pm$ on $\Sigma=\partial M$ is exactly the setwise difference between $S$ and the subpages $P$ and $h(P)$, and the product partial foliated open book was constructed so that $S$ is  built up from $P$ (respectively, $h(P)$) via sequence of handle additions, one corresponding to each hyperbolic point in $R^+$ (respectively, $R^-$) as $t$ increases.  Thus the result is an $S^1$-family of pages identified along $B$ whose topology changes by a single $1$-handle addition or saddle resolution at each $t$-value corresponding to a hyperbolic point on the foliated boundary.  Equivalently, there is a \jel{smooth} map from $M\!\smallsetminus\! B\rightarrow S^1$ with only isolated critical points, each located on $\partial M$, so \jel{we may perturb this to an $S^1$-valued Morse function on the complement of the binding.} 
 

Since both the original and new boundary surfaces are divided by $\Gamma$, we may isotope the contact structures in a neighborhood of the gluing surface to agree. Furthermore, the product partial foliated open book supported an $I$-invariant contact structure, so the contact structure supported by the new glued manifold is contactomorphic to the contact structure supported on the original partial open book, as desired.  \vv{We have to clean this up a bit}
\end{proof}

In fact, Proposition~\ref{prop:fpluspf} is the key ingredient in proving that every contact manifold whose boundary has an $S^1$-Morse foliation admits a compatible foliated open book.

\begin{proof}[Proof of Theorem~\ref{thm:exist1}] Given $(M, \xi, \mathcal{F})$, choose a partial open book with $\Gamma$ dividing $\mathcal{F}$.  Then apply Proposition~\ref{prop:fpluspf}.
\end{proof}

\subsection{Sorted foliated open books}
In this section we describe a topological condition between cutting arcs  and attached handles on the pages of a foliated open book $(B, \pi, \mathcal{F})$, which allows us to decompose a foliated open book as a union of a partial open book and the partial foliated open book $I(\partial M,\F,\Gamma)$.

Let $(B,\pi,\F_\pi)$ be a Morse foliated open book compatible with $(M,\xi,\F_\xi)$ and fix a gradient-like vectorfield $\nabla \pi$ so that the restriction of its flows 
 to $\partial M$ on an elementary tile is as shown in Figure~\ref{fig:grad}. \marginpar{\vv{probably phrase it in words for added readibility.., also define elementary tile earlier!}}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{gradient}
\caption{ $\nabla \wtpi$ shown in purple on an elementary tile of $\mathcal{F}$. }\label{fig:grad}
\end{center}
\end{figure}

%As usual, we blow up $B$ to $B\times S^1$ \marginpar{\vv{$S^1\times B$ or $B\times S^1$?}} to obtain $M'$, and we extend $\pi$ to $M'$ continuously. We will additionally cut open $M'$ along $\pi^{-1}(0)$, again extend $\pi$ continously to get a cobordism $M''$ with a Morse function $\pi\colon M''\to [0,1]$. 
As in subsection \ref{ssec:afob} we can consider  the ascending and descending manifolds $W_{p_i}^-$ and $W_{p_i}^+$ with respect to $\nabla \pi$ for each critical point $p_i$ of $\pi$.  

\begin{lemma}\vv{Will we use this?} Let be a neighborhood of the union of the descending gradient flow lines from any  positive hyperbolic point with critical value less than $t$; 
the ascending gradient flow lines from any  negative hyperbolic point with critical value less than $t$; and  the leaf $\wtpi^{-1}(t)$:
\[R_t=\big[ \bigcup_{\text{ind}(p)=2, \pi(p)<t} N(W_p^+)\big] \cup \big[\bigcup_{\text{ind}(p)=1, \pi(p)<t} N(W_p^-)\big] \cup \big[ N(\wtpi^{-1}(t) )\big].\]
\jel{I put in the proper notation, but I prefer the version without it.}
Then $R_t$ is homeomorphic to $R^+$. 
\end{lemma}

\begin{proof} (Easy to see this for $t=0$, then show passing through a hyperbolic point preserves the neighborhood.)
\end{proof}

\begin{definition}\label{def:sorted} %A foliated open book is \emph{sorted} if the ascending manifold $W_p^+$ for each index 1 critical point $p$ and the descending manifolds $W_q^-$ of each index 2 critical point $q$ are disjoint in $M''$.

A foliated open book is \emph{sorted} if the manifolds $W_p^+$ ascending from each index 1 critical point to $\pi^{-1}(0)$ and the manifolds $W_q^-$ descending from each index 2 critical point to $\pi^{-1}(0)$ are disjoint in $M\!\smallsetminus\! \pi^{-1}(0)$.  
\end{definition}




\begin{proposition}\label{prop:makepfob} If  $(B,\pi, \mathcal{F})$ is sorted, then it decomposes as a partial open book glued to a product partial foliated book for  $(\partial M,\mathcal{F})$.
\end{proposition}

\vv{I think what you describe here, is the other direction, which could also be in a proposition if we want to} As an indication of why this proposition is plausible, consider a partial open book $(S, P, h)$.  Transforming $S$ into $P$ requires cutting along a collection of arcs, and then transforming $P$ into $S$ involves adding a collection of handles.  If these operations are grouped at $S=\{0, \pi\}$, the result is a partial open book.  On the other hand, if each cut and each one-handle addition is assigned a distinct $t$-value, then the result is an abstract foliated open book with $S_k=P$.   A sorted foliated open book is more general, however, as it does not require all the cuts to happen before all the handle additions. 
\vv{Do you wanna say something, that in this case we can rearrange everything as we please?}

\jel{We are building $S$ from $P$ by $1$-handle addition, not building $S$ from $S\!\smallsetminus\! P$ by 1-handle addition.}



\begin{proof}[Proof of Proposition~\ref{prop:makepfob}]
Let $(M, \xi, \Gamma)$ be a contact manifold with a compatible sorted foliated open book $(B, \pi, \mathcal{F})$.  We will identify a partial open book for $(M, \xi, \Gamma)$  in the interior and show that the setwise difference between the original and new manifolds is a product partial foliated open book for $(\partial M, \mathcal{F})$.

Choose $\varepsilon$ sufficiently small so that $[-\varepsilon, \varepsilon]$ contains no critical values and choose a subinterval $B'$ contained in an open subinterval of each component of $B$. Let $N$ be a flow-invariant neighborhood of $\partial M\cup \big(\bigcup_{p_i \text{critical}} N(p_i)\big)$  in $M\!\smallsetminus\! S_0$.  
We further require that $N\cap B=B\!\smallsetminus\! B'$.   Here $N(p_i)$ denotes a neighborhood of the $i^{th}$ critical point, so a flow-invariant neighborhood of this ball is in fact is a neighborhood of $W_{p_i}^+\cup W_{p_i}^-$.  Let $N'$ be a neighborhood of $\partial M$ with the properites that $N\cap B=N'\cap B$, but away from $B$, there exists an open neighborhood of $N'$ contained in $N$. \vv{wait, isn't $N'$ open?}

We make one modification to the neighborhoods constructed so far: on  $S_\varepsilon \cap R^+$, compress \vv{what does compress mean? Make it smaller? or factor?} $N\cup N'$ \vv{Why do you take the union, if it's already contained?} to contain only the positive half of the leaf $\wtpi^{-1}(\varepsilon)$ and on $S_{\-\varepsilon}\cap R^-$, compress $N\cup N'$ to contain only the negative half of the leaf $\wtpi^{-1}(-\varepsilon)$.  
Define $\Phi$ to be the manifold which agrees with $N$ for $\varepsilon \leq t\leq 2\pi-\varepsilon$ and equals $N'$ for $-\varepsilon <t<\varepsilon$. Note that $\Phi$ is not a manifold with boundary because  the intervals of $\wtpi^{-1}(\pm \varepsilon)$ do not have neighborhoods.  Define $\Pi$ to be $M\!\smallsetminus\! \Phi$.

We claim that $\Phi$ decomposes as a partial open book for $M$ and that $\Phi$ decomposes as a foliated open book for $(\partial M, \mathcal{F})\times I$.

Since $\Phi$ is  homeomorphic to a quotient of $\partial M\times I$ that collapsed subsets of $\wtpi^{-1}(\pm \varepsilon) \times I$ to curves,  it follows that  $\Pi$ is homeomorphic to $M$.  We show that it is naturally equipped with the structure of a partial open book $(S'', P'', h)$.  For $-\varepsilon\leq t\leq \varepsilon$, define $S'':=S_t \cap \Pi=S_t\!\smallsetminus\! N'$.   The remaining $\Pi \cap [\varepsilon, 2\pi-\varepsilon]$ is a homeomorphic to a product $P'\times  [\varepsilon, 2\pi-\varepsilon]$, as the topology of the original pages changed only at critical $t$ values and neighborhoods of their ascending and descending manifolds are in $\Phi$.  By construction,   $R^+=\big(S'' \times\{\varepsilon\} \big)\!\smallsetminus\! P''= \partial \Phi\cap \partial \Pi \cap \pi^{-1}(\varepsilon)$ is homeomorphic to a neighborhood of the postive separatrices of positive hyperbolic points.  Similarly,  $R^-=S_{-\varepsilon}\!\smallsetminus\! P''= \partial \Phi\cap \partial \Pi \cap \pi^{-1}(-\varepsilon)$ is homeomorphic to a neighborhood of the negative separatrices of negative hyperbolic points.    The product foliation on $P''\times[\varepsilon, 2\pi-\varepsilon]$ will be determined by $\Phi$, which we examine next.


The manifold $\Phi \cong \partial M \times I$ evidently has two boundary components, one of which --- the \textit{outer boundary}--- is the original foliated boundary of $M$, while the other  --- the \textit{inner boundary}--- is shared with $\Pi$.  (Note that these coincide along parts of $\wtpi^{-1}(\pm \varepsilon)$. )The latter has horizontal components which are subsets of $S_0$ and coincide with $R^\pm$ on the partial open book $\Pi$.  %For convenience, blow up each component of $B$ to a cylinder $B\times S^1$.  
For $t\in [-\varepsilon, \varepsilon]$, we have that $S'_t:= \Phi\cap S_t$ is a rectangle connecting two components of $B\!\smallsetminus\! B'$ with opposite signs.  This portion of the inner boundary of $\Phi$ is therefore  foliated by line segments whose endpoints meet at points in $E$.  We call these the $P$-bigons, and  adjacent to each $P$-bigon on the inner boundary of $\Phi$ is the copy of $R^\pm$ shared with $\Pi$.  Each remaining component of the inner boundary is a topologically a disc, and %, and in fact, these discs are the remaining bigons foliated by $\mathcal{G}_{2\pi-s, t}$ as in the construction of the product partial foliated open book.  
we will construct the $\mathcal{G}_{2\pi-\varepsilon, t}$ foliation in the complement of the $P$-bigon on the inner boundary component.  Figure~\ref{fig:print} indicates the essential properties of the $t=\varepsilon$ leaf, which is shown in pink. Each component of the leaf starts at a positive elliptic point on the inner boundary component and runs along the boundary of $P_\varepsilon$ until its intersection with $\Gamma$.  It then runs along the boundary of $N\cap S_\varepsilon$ until it reaches the next negative elliptic point in the inner boundary.  Construct the analogous curve \jel{specify!} on $S_{-\varepsilon}$ and then extend $\mathcal{G}_{2\pi-\varepsilon}$ across each bigon.  Note that this portion of the foliation specifies an parameterization as  $\partial P\times [-\varepsilon, \varepsilon]$ on $\Pi$, as promised earlier.  Extend this into $P\times [-\varepsilon, \varepsilon]$ to complete the construction of the partial open book.  


\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.9]{printing}
\caption{ The pink curve is $\mathcal{G}_{2\pi-\varepsilon, \varepsilon}$ \jel{fix}}\label{fig:print}
\end{center}
\end{figure}

Using the identification of $\Phi=\partial M\times I$, extend $\mathcal{G}$ to the rest of $\Phi$ as in Figure~\ref{fig:prodpfpob}.  Note that for $s<2\pi-\varepsilon$, the curves in $\mathcal{G}_{s,t}$ that survive in the product partial foliated open book are all subcurves of $\mathcal{G}_{2\pi-\varepsilon}$, so no further choices are required.  Once $\mathcal{G}$ and $\mathcal{F}$ are printed on every layer, the decomposition of $\Phi$ into pages follows, and by construction, these pages glue to those of $\Pi$. Since the  contact structure supported by $\Phi$ is $I$-invariant, we may cut along the inner boundary to separate $M$ into a partial and product partial foliated open book.  \jel{Last sentence doesn't make sense.}

\end{proof}




\jel{If some boundary component is a sphere foliated by parallel arcs, then there are no handles.  How do  the two different types of bigons connect the two elliptic points?}


\begin{proposition}\label{prop:disj}
A foliated open book $(B,\pi,\Fob)$ may be stabilized to a sorted foliated open book.
\end{proposition}

\begin{proof}  \vv{checked 05.04}
Using the notation of subsection \ref{ssec:afob} we choose regular values $t_i$ between the critical values $t_i'$ so that with respect to the cyclic order on $S^1$ we have $t_0<t_1'<t_1<\cdots<t_{2k-1}<t_{2k-1}'<t_2k<t_0$. Then $S_i=(\pi')^{-1}(t_i)$ are surfaces with boundary $\alpha_i=\partial M\cap S_i$ union $B\times\{t_i\}$ and corners at $B\times\{t_i\}\cap\alpha_i$. In general denote by $S_t=\pi^{-1}(t)$ and $\alpha_t=\partial M\cap \pi^{-1}(t)$.
\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.5]{morse}
\caption{Left: a 3-manifold $M$ with boundary, and foliated open book $(B,\pi,\Fob)$, the binding is marked with blue, while the properly embedded surface $\pi^{-1}(0)$ is yellow. Right: the corresponding $M'$, $V$ is on the right, $\partial^\pm M$ is on the top and bottom and $B\times I$ is the vertical boundary on the left hand side.   
}\label{fig:morse}
\end{center}
\end{figure}
For a critical point $p_i$ with $\pi(p_i)=t_i'$ let $W_{p_i}^{-}$ denote its descending manifold, that intersects $S_{i-1}$ in a properly embedded arc $\gamma_{i-1}$ with boundary on $\alpha_{i-1}$ or in 2 points $r_{i-1},q_{i-1}\in\alpha_{i-1}$. Similarly let $W_{p_i}^+$ denote ascending manifold of $p_i$.
%
%
% 
%Suppose that $0$ is a regular value of $\pi$, we will work with the Morse function $\overline{\pi}\colon M' \to [0,2\pi]$, where $M'$ is the closure of $M\!\smallsetminus\! \overline{\pi^{-1}(0)}$, and $\overline{\pi}$ is the continuous extension of $\pi\vert_{M\!\smallsetminus\! \overline{\pi^{-1}(0)}}$ to $M'\!\smallsetminus\! B$. The manifold $M'$ is a manifold with boundary and corners, as on Figure \ref{fig:morse}. The boundary is the union of $V$ that is the closure of $\partial M\!\smallsetminus\! \partial \overline{\pi^{-1}(0)}$, $B\times [0,2\pi]$,  $\partial^-M'=\overline{\pi}^{-1}(0)$ and $\partial^+M'=\overline{\pi}^{-1}(2\pi)$. The 1-codimensional corners of $M'$ are the intersections $V \cap \partial^-M'$, $V\cap \partial^+M$, $B\times\{0\}$ and $B\times \{2\pi\}$.
%The 2-codimensional corners are $\partial B\times \{0\}$ and $\partial B\times \{2\pi\}$.
%Let $S_t$ be the level set $\overline\pi^{-1}(t)$. For regular values $S_t$ is surface with boundary and corners. The boundary of $S_t$  is the union of  $B\times \{t\}$ and $E_t=(\overline\pi\vert_V)^{-1}(t)$, and its corners are at $\partial B\times \{t\}$. The leaves of the foliation $\Fob$ on $V$ are given by $E_t$, thus by assumption each component of $E_t$ is an interval.
%
%
%
%Choose a gradient-like vectorfield $X$ for $\overline\pi$. Recall, that by the definition of foliated open books the function $\overline{\pi}$ only has index 1 and 2 critical points, that are index 1 critical points of $\overline\pi\vert{V}$. This means that for an index 1 critical point $q$ the stable manifold $W^+_q$ of $X$ is an interval properly embedded into $V$ with endpoints on $\overline\pi^{-1}(0)$, while the unstable manifold  $W^-_p$ for $X$ is an embedded half disc. Similar description applies for the stable and unstable manifolds of an index 2 critical points $p$ of $\overline\pi$. 
See Figure \ref{fig:morse2}.

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.3]{morse2}
\caption{Stable and unstable manifolds of critical points of $\overline{\pi}$}\label{fig:morse2}
\end{center}
\end{figure}

We will cut open $M'$ along $S_0$, and consider the restriction $\pi_0$ of $\pi$ to $\overline{M'\!\smallsetminus\! S_0}$ into $[0,1]$.
In the following we will prove that by choosing the gradient-like vectorfield $X$, and possibly stabilising the foliated open book $(B,\pi,\Fob)$ we can achieve that none of the stable manifolds $W_{p_i}^+$ of index 2 critical points of $\pi_0$ intersect none of the unstable manifolds  $W_{p_j}^-$  of index 1 critical points of $\pi_0$. Note that we need to cut open $M'$ to avoid the wrapping of $W_p^\pm$ in the $S^1$-direction.

Fix a pair of index 1 and index 2 critical points $p_i$ and $p_j$ with $i<j$, and  assume, that for any critical point $p_l$ for $i<l<j$ of index 1 (or 2) we have $W_{p_l}^-\cap W_{p_i}^+=\emptyset$ (or $W_{p_j}^-\cap W_{p_l}^+=\emptyset$). %Note that since  $\pit_0=\pi_0\vert_{\partial M}$ is Morse--Smale and $p_i$ and $p_j$ are both index 1 critical points of $\overline\pi\vert_{\partial M}$ we have that $W_{p_i}^+\cap \partial M$  is disjoint from $W_{p_j}^-\cap \partial M$.  
Fix a regular level $t$ between $t_i'$ and $t_j'$, then by possibly adding some $-T\alpha_{t'}$ (for $t_i'<t'<t$) to the gradient like vectorfield $X$ we can make sure that with respect to the boundary orientation of $S_t$ the points 
$W_{p_j}^-\cap {\alpha_t}$ and $W^+_{p_i}\cap \alpha_t$ are all different and 
none of the two points of $W_{p_j}^-\cap\alpha_t$ are before points of $W^+_{p_i}\cap \alpha_t$.

Choose the arc $\gamma$ on $S_t$ that starts on $B\times\{t\}$, follows the orientation of $\alpha_t$ until it reaches the endpoint of $W^+_{p_i}\cap \alpha_t$ on $\alpha_t$ (this is possible, because all components of $\alpha_t$ are arcs), then follows $W^+_{p_i}\cap S_t$ entirely, lastly it ends on $B\times \{t\}$ this time by following the opposite orientation of $\alpha_t$. By the condition on the starting points of $W_{p_j}^-\cap \alpha_t$ and $W^+_{p_i}\cap \alpha_t$ we see that $\gamma$ intersects $W^-_{p_j}\cap S_t$  exactly as $W^+_{p_i}\cap S_t$. See the first picture of Figure \ref{fig:gamma}.

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.4]{dehn}
\caption{Gamma.}\label{fig:gamma}
\end{center}
\end{figure}

Now we construct the abstract foliated open book $(\{S_i'\},h')$ from $(\pi,B,\Fob)$ by cutting it at time $t$, so $S_0'=\pi^{-1}(t)$. Note that this is a ``rotation'' of the pages $\{S_i\}$, and thus $h'$ is (some sort of) conjugation, of what the gradient flow would induce between $S_{2k}$ and $S_0$. 

Next we perform a stabiliztaion of $(\{S_i'\},h')$ along the arc $\gamma$. Going back to the embedded language this gives us a new open book $(B_{{st}},\pi_{{st}})$, with the same critical points and $W^+_{p_i}(\pi_{st})\cap\pi_{st}^{-1}(t)=W^+_{p_i}\cap S_t$  but $W^-_{p_j}(\pi_{st})\cap\pi_{st}^{-1}(t)=D_{\overline{\gamma}}(W^+_{p_i}\cap S_t)$. 
(here we parametrised $\pi_{st}^{-1}(t)$ as the stabiiasation of $S_0'$). As it is shown on the right hand side of Figure \ref{fig:gamma} we get that $W^+_{p_i}(\pi_{st})\cap\pi_{st}^{-1}(t)$ is disjoint from $W^-_{p_j}(\pi_{st})\cap\pi_{st}^{-1}(t)$, thus the corresponding ascending and descending manifolds are disjoint too.  During this process we did not introduce extra intersection points for other pairs of critical points, so we can continue our method to remove all intersections. 
\end{proof}

\vv{I commented out something that is not needed anymore, check it before you erease..}
%One may easily detect whether an abstract foliated open book is sorted.  Starting from $S_0$, each time $S_{i+1}$ is formed from $S_i$ via a handle addition, decorate all subsequent surfaces with  the co-core of the handle.  Now suppose that $S_{i+1}$ is formed from $S_i$ by cutting along some arc.  Decorate all previous pages with the cutting curve.  The next lemma follows immediately from Definition~\ref{def:sorted}.
%
%\begin{lemma} An abstract foliated open book is sorted if the co-cores of added handles and the cutting arcs are disjoint on $S_t$ for all $t\neq 0$. 
%\end{lemma}
%
%
%\begin{proof}[Proof of Proposition~\ref{prop:disj}]
%Beginning from $S_0$, we add one curve to the surface at each step.  If an added curve violates the disjointness condition, we will describe how to stabilize the open book so that the curves remain disjoint.  
%
%
%Consider a cutting arc $\alpha$. Since we allow cutting arcs to slide along the $\alpha_i$ in the complement of $B$, we may assume that there is no endpoint of $\alpha$ between  endpoint of any cocore.
%\jel{finish this}
%\end{proof}





\begin{example} \jel{Explain the relationship between 2 PFOBs compatible with the same POB?  (i.e., same $\Gamma$ but different $\mathcal{F}$).  The answer is that we have two PFOBs for $\Sigma\times I$ glued along their P sides to give a new FOB for $\Sigma \times I$.  }
\end{example}

\begin{question} Are there local moves between $(\mathcal{F}_i, f_i)$ $i=1,2$ for the same $\Gamma$?
\end{question}



